Trace-Relating Compiler Correctness and Secure Compilation

Compiler correctness is, in its simplest form, defined as the inclusion of the set of traces of the compiled program into the set of traces of the original program, which is equivalent to the preservation of all trace properties. Here traces collect, for instance, the externally observable events of each execution. This definition requires, however, the set of traces of the source and target languages to be exactly the same, which is not the case when the languages are far apart or when observations are fine-grained. To overcome this issue, we study a generalized compiler correctness definition, which uses source and target traces drawn from potentially different sets and connected by an arbitrary relation. We set out to understand what guarantees this generalized compiler correctness definition gives us when instantiated with a non-trivial relation on traces. When this trace relation is not equality, it is no longer possible to preserve the trace properties of the source program unchanged. Instead, we provide a generic characterization of the target trace property ensured by correctly compiling a program that satisfies a given source property, and dually, of the source trace property one is required to show in order to obtain a certain target property for the compiled code. We show that this view on compiler correctness can naturally account for undefined behavior, resource exhaustion, different source and target values, side-channels, and various abstraction mismatches. Finally, we show that the same generalization also applies to many secure compilation definitions, which characterize the protection of a compiled program against linked adversarial code.

==> app-proofs-marco.tex <==
% !TEX root = ./main.tex


\section{Proofs for \Cref{SEC:MARCO}}\label{sec:proofs-marco}

\begin{proof}[Proof for \Thmref{thm:inst-marco-gensend}]
	We proceed by induction on \src{\tau} and then by induction on \src{\tau'}:
	\begin{description}
		\item[$\src{\tau}=\src{N}$ and $\src{\tau'}=\src{N}$]

		By canonicity we have that $\src{v} = \src{\pair{n,n'}}$.

		\gensend{\cdot}{\cdot} translates that into \trg{\sendt{n};\sendt{n'}}.

		By \Cref{tr:e-tm-send}, that produces $\trg{Q}=\trg{n;n'}$.

		We need to prove that $\src{\pair{n,n'}}\sim\trg{n;n'}$, which holds by \Cref{tr:tr-rel-n}.

		\item[$\src{\tau}=\src{N}$ and $\src{\tau'}=\src{\tau_1\times\tau_2}$]

		Analogous to the other cases, by IH and \Cref{tr:tr-rel-n-m}.

		\item[$\src{\tau}=\src{\tau_1\times\tau_2}$ and $\src{\tau'}=\src{N}$]

		Analogous to the other cases, by IH and \Cref{tr:tr-rel-m-n}.

		\item[$\src{\tau}=\src{\tau_1\times\tau_1'}$ and $\src{\tau'}=\src{\tau_2\times\tau_2'}$]

		So by canonicity $\src{v}=\src{\pair{\pair{v_1,v_1'},\pair{v_2,v_2'}}}$.

		By definition of \gensend{\cdot}{}:
		\begin{align*}
			&
			\gensend{\compm{\src{\Gamma\vdash \pair{\pair{v_1,v_1'},\pair{v_2,v_2'}} : \tau\times\tau'}}}{\tau\times\tau'}
			\\
			=&\
			\trg{\gensend{\compm{\src{\Gamma\vdash \pair{v_1,v_1'} : \tau}}}{\tau};\gensend{\compm{\src{\Gamma\vdash \pair{v_2,v_2'} : \tau'}}}{\tau'}}
		\end{align*}

		Since \trg{\gensend{\compm{\src{\Gamma\vdash \pair{v_1,v_1'},\pair{v_2,v_2'}: \tau\times\tau'}}}{\tau\times\tau'} \Xtot{Q_1;Q_2} 0}, by IH we have
		$\src{\pair{v_1,v_1'}}\sim\trg{Q_1}$
		and
		$\src{\pair{v_2,v_2'}}\sim\trg{Q_2}$.

		We need to prove that $\src{\pair{\pair{v_1,v_1'},\pair{v_2,v_2'}}}\sim\trg{Q_1;Q_2}$, which holds by \Cref{tr:tr-rel-m-m}, for $\src{M}=\src{\pair{v_1,v_1'}}$ and $\src{M'}=\src{\pair{v_2,v_2'}}$.
		\qedhere
	\end{description}
\end{proof}

\begin{proof}[Proof for \Thmref{thm:inst-marco-cc}]
	By definition we need to prove that
	$$\forall\src{t},\src{\tau},\trg{Q}. \ift \trg{\compm{\src{\srce\vdash t:\tau}}\sem\trg{Q}} \thent \exists\src{Q}\sim\trg{Q} \andt \src{t\sem Q}$$
	We proceed by induction on the typing derivation of \src{t}.
	\begin{description}
		\item[Base.]
		\begin{description}
			\item[$\src{t}=\src{n}$]
			Trivial, by \Cref{tr:tr-rel-empty} as no trace is emitted.
		\end{description}
		\item[Inductive.]
		\begin{description}
			\item[$\src{t}=\src{t'\op t''}$]
			By IH.
			\item[$\src{t}=\src{\iftes{t'}{t''}{t'''}}$]
			By IH.
			\item[$\src{t}=\src{\letins{x}{t'}{t''}}$]
			By IH.
			\item[$\src{t}=\src{\pair{t',t''}}$]
			By IH.
			\item[$\src{t}=\src{\projone{t'}}$]
			By IH.
			\item[$\src{t}=\src{\projtwo{t'}}$]
			By IH.
			\item[$\src{t}=\src{\sends{t'}}$]
			By IH we have that if \trg{\compm{\src{\srce\vdash t:\tau}}\sem\trg{Q}} then $\exists\src{Q}\sim\trg{Q}$ and \src{t\sem Q}.

			By definition of \compm{\cdot} and of $\trg{\sem}$ we need to prove that if
			\begin{align*}
				\trg{
					\letint{
						x
					}{
						\compm{\src{\Gamma\vdash t:\tau\times\tau'}}
					}{ \gensend{x}{\tau\times\tau'} }
				}
				\Xtot{Q}
				\trg{\_}
			\end{align*}
			Then $\src{\sends{t}\Xtos{Q}\_}$ and $\src{Q}\sim\trg{Q}$.

			The reductions proceed as follows:
			\begin{align*}
				&
				\trg{
					\letint{
						x
					}{
						\compm{\src{\Gamma\vdash t:\tau\times\tau'}}
					}{ \gensend{x}{\tau\times\tau'} }
				}
				\\
				\Xtot{Q'}
				&
				\trg{
					\letint{
						x
					}{
						\compm{\src{\Gamma\vdash v:\tau\times\tau'}}
					}{ \gensend{x}{\tau\times\tau'} }
				}
				\\
				\redt
				&
				\gensend{\compm{\src{\Gamma\vdash v:\tau\times\tau'}}}{\tau\times\tau'}
				\\
				\Xtot{Q''}
				&
				\trg{0}
			\end{align*}
			In the source we have $\src{\sends{t}} \Xtos{Q'} \src{\sends v} \Xtos{v} \src{0}$.

			By IH we have that $\src{Q'}\sim\trg{Q'}$.

			By \Cref{tr:tr-rel-full}, to prove that $\src{Q';v}\sim\trg{Q';Q''}$ we need to prove that $\src{v}\sim\trg{Q''}$.

			By \Thmref{thm:inst-marco-gensend} we have that $\src{v}\sim\trg{Q''}$, so this case holds.
			\qedhere
		\end{description}
	\end{description}
\end{proof}

==> criteria.tex <==
\section{Robust Part} \ca{just temporary title}
\label{sec:diagram}

\ca{diagram updated up to subset-closed hyperproperties, for relational properties the plan
    is to use alternative characterizations of the property-full criteria. For instance
    $\rtrtp$ can be expressed in terms of pairs of trace properties. }

\ca{TODO: provide all definitions}

\input{robust_diagram}

==> diagram.tex <==
\begin{figure}
  \centering
\begin{tikzpicture}[scale = 0.70]
	%\begin{pgfonlayer}{nodelayer}
		\node  (0) at (0, 5  )  {\hyperP $\small{\iff}$ \pf{\hyperP}};
		\node  (1) at (0, 2.5)  {\traceP $\small{\iff}$ \pf{\traceP}};
		\node  (2) at (0, 0)    {\safetyP $\small{\iff}$ \pf{\safetyP}};
	%\end{pgfonlayer}
	%\begin{pgfonlayer}{edgelayer}
		\draw [->] (0) to (1);
		\draw [->] (1) to (2);
	%\end{pgfonlayer}
\end{tikzpicture}\ch{Could put something like this in Section 4}
    \caption{Relative strength order of criteria for Hyperproperties,
             Trace Properties and Safety Properties preservation
             with same observable events for source and target}\label{fig:diagram}
\end{figure}
\medskip


==> diff_traces.tex <==
% !TEX root = ./rc.tex
\section{Differing Source and Target Trace Models}
\label{sec:different-traces}

So far we have assumed that the source and target languages share the
sets of traces and properties.
%
This is a reasonable assumption if observable events are coarse enough
to be common to the source and target language (\EG as it happens
CompCert~\cite{Leroy09}).
%
There are various settings in which this assumption does not hold though:
\ca{maybe we can write here the whole list we had on the board}
\begin{itemize}
\item when values appear in traces and the source and target don't
  share the same notion of values~\cite{PatrignaniG17};
\item when the source language has ``undefined behavior'', which is a
  special event only occurring in source traces, and which leads to
  an arbitrary trace continuation in the target~\cite{Leroy09};
\item when the target language has more events because it is the
  target of multiple source languages;
\item when traces model observations that could become more precise at
  lower levels, \EG because of side-channels like
  timing~\cite{CostanzoSG16};\ch{But with traces formed of such
    leakages even compiler correctness is hopeless~\cite{BartheGL18},
    even more our extensions of it to adversarial contexts!  So maybe
    this is not such a great example after all. The only kind of work
    that could fit here is the one by Zhong Shao~\cite{CostanzoSG16},
    where the source and target observations are different, but still
    equivalent. So started watering this down by adding a ``could'' above.}
\item in general, when there is a big difference between the
  abstractions of the source and target languages.
\end{itemize}

% \MP{ there's other reasons too: again, the target may talk about more
%   things, because it's a compilation target for multiple languages and
%   the source is a language designed with a specific abstraction in mind. }

% \rb{I would also try to give a general description of causes for the divergence
% and then some examples, like you have now.}
%
% \ch{I find this bijection story a confusing digression,
%   but would still like to understand why would it be relevant here}%
% Using standard set-theoretical arguments we know that, if the two sets of events are both finite or in a bijection,
% then so are the sets of traces and properties. In general such a bijection between traces is not constructive,
% so that it is interesting to study variants of our criteria handling the discrepancies between trace events.
% In this section we focus on \rtp and \pf{\rtp}, leaving a generalization to the remaining criteria as future work.

% \MP{ latex guideline: the \textbackslash\textbackslash\ is not meant to be used in text, it often breaks things}

In this section, typographic conventions for source and target elements extend
to properties, previously common to both levels. We will denote with \tS{s} and \tT{t} source and
target traces respectively. \ca{any other proposal is welcome, just modify macros in cmd.tex}
%
The criteria we are going to study regard the preservation of trace properties,
safety properties and hyperproperties. In case source and target traces coincide they
can be classified according to \Cref{fig:diagram} and expressed in terms of their corresponding
\emph{property-free} equivalent. \ca{TODO: explain that these comprehends also relational hprop etc.}
%
\input{diagram}
%
Let us temporarily focus on the preservation of satisfaction of arbitrary trace properties, $\tp$ and
its equivalent ``property-free'' characterization $\pf{\tp}$.

  \begin{align*}
    \tp: \quad
    \forall \pi \in 2^{\ii{Trace}}. ~\forall \src{W}.~
    &
      (\forall t \ldotp \src{W \sem} t \Rightarrow t \in \pi_S)
      \Rightarrow
    \\
    &
      (\forall t \ldotp \cmp{W} \trg{\sem} t \Rightarrow t \in \pi_S)
    \\
    \\
     \pf{\tp}: \quad
     \forall \src{W} ~\forall t \ldotp \cmp{W} \trg{\sem} t \Rightarrow \src{W \sem} t
    \\
  \end{align*}


==> early-failure.tex <==
% !TeX root = main.tex
In this section, we describe two kind of relations between traces that capture
the compiler correctness theorems that are present in two modern verified compilers,
CompCert~\cite{Leroy09}, and CakeML~\cite{TanMKFON19}.

In CompCert's trace model, an execution can end in an undefined behavior.
CompCert allows compiled program to produce traces that ``improve'' over source
traces, that is traces that are the same as the source ones, except they are
allowed to replace a possible undefined behavior by anything.
%
To model CompCert, we introduce an undefined behavior relation
(\autoref{sec:example-undef}) that allows relating a target trace and the same
trace at the source level, or a target trace and any of its prefix, followed by
an undefined behavior in the source.

In CakeML, the source language is a ML-like language without notions such
as memory or resources. However, this notions can not be ignored anymore when
compiling down to lower-level languages.
%
The CakeML compiler's theorem accounts for the possibility of memory exhaustion
by allowing compiled programs to end early due to memory exhaustion.
%
We capture CakeML's behavior by introducing a resource-exhaustion relation
(\autoref{sec:example-resources}) that relates a source trace and the same
trace at the target level, or a source trace and any of its prefix, followed by
a memory exhaustion error in the target.

In the following examples, we will consider source traces in \(\src{\mathcal{S}}\) and
target traces in \(\trg{\mathcal{T}}\) composed of the same events from a set \(\Sigma\),
% \MP{ you coloured them below, why not here?}\jt{because I forgot}
with the exception that one of the source or the target also has a new special
terminal event, either \eundefS, or \oomT,
that mark the failure (undefined behavior or memory exhaustion).



% \ch{\(\mathcal{S}\) and \(\mathcal{T}\) have to be quite close to each other
%  to allow common prefixes, no?}
% \jt{yes}


==> instance-marco-inputs.tex <==
% !TEX root = ./main.tex
\subsubsection{Possible Extensions: Inputs}

\mbox{}\et{not sure what the point of this subsection is. There does not seem to be anything to put forth as such}
\MP{
	at some point we discussed whether we should add inputs,
	these are my thoughts on why adding inputs is not necessary and does not lead to necessarily new insights.
	I expect this will be moved to the appendix.
}

This section considers the addition of another source of trace events to the languages: inputs.
We have different ways to model inputs, though we argue that none of them add insights beyond what already developed.
\begin{enumerate}
	\item \Sm inputs \src{N} and \Tm inputs \trg{N}.

	In this case the source program must already contain the code to ``compose'' the inputs into larger data structures (\IE into larger pairs).
	Compiling such a program adds nothing to what already provided.

	\item \Sm inputs \src{\tau\times\tau} and \Tm inputs \trg{N};

	In this case the source program handles inputs as pairs while the target handles them as single naturals.
	Necessarily, the compiled program must therefore contain additional instructions to compose a pair such as the source one starting from individual naturals.
	This is the dual case of the compilation of output, so it adds no particular insight.
	Instead of having \gensends{\cdot}, we would need another function that \emph{relying on the type information} (which is available through compilation), builds a target pair that behaves like the source level one.

	\item \Sm inputs \src{N} and \Tm inputs \trg{\tau\times\tau};

	In this case the target seems more expressive than the source
	How can we compile a ``\src{read}~\src{n}'' into a ``\trg{read}~\trg{\pair{n',n''}}''? \et{just \trg{read}~\trg{\pair{n',0}}? (by analogy with the out case below)} \MP{except that inputs come from the environment and we have no control over how they are shaped}

	On one hand, this seems orthogonal to also having outputs, it's more of an issue of how to treat inputs.
	In fact, if we did the opposite of the above, so output \src{N} in \Sm but output \trg{\tau\times\tau} in \Tm,
	we would compile ``\src{out~n}'' into ``\trg{out~\pair{\compm{n},0}}''.

	More generally, thus, the issue is how to deal with inputs.
	Typically, the code after the read will have to case it in case we need to react to specific inputs.
	That code will also be present in the compiled code (it comes from the source), but the issue would be: what element of the pair should we pick in the target?
	If the target pair models a multiple input port with different quality of value, it may be worth to consider a backtracking approach, \IE we compute with the first projection and if that fails, we backtrack and continue with the second.
	However, this seems vastly orthogonal to the issue of relating traces, it's more of a system design issue.

	Thus, this option is also not leading to any particularly interesting case (w.r.t. cross-trace relations at least).

	\item \Sm inputs \src{\tau\times\tau} and \Tm inputs \trg{\tau\times\tau};

	In this case there is no abstraction gap, so adding inputs does not lead to any particularly interesting case.
\end{enumerate}


==> instance-more-target.tex <==
% !TEX root = ./main.tex

This example shows how to relate programs where a single source action gets mapped to multiple target ones.
To illustrate this, we use a source language that performs network communication but that does not have a notion of network packet.
On the other hand, the target language has a notion of packets, which have a fixed size.
Thus, the source has a single action of the form \sends{v1,v2,v3}, which means to send content \src{v1,v2,v3} over the network.
Such an action gets related to a whole target trace \sendt{v1}, \sendt{v2}, \sendt{v3}, which corresponds to sending content \trg{v1,v2,v3}.

For simplicity, we carry out this example without implementing a real concurrent interface for sending over the network since this is orthogonal to the point we want to make.


\subsubsection{\Sm: Source}
\Sm is a statically-typed language with simple types (natural numbers and pairs) whose syntax is presented below.
The key aspect of \Sm is the primitive for sending \emph{pairs} over a network interface.
\begin{align*}
	% \src{P} \bnfdef
	% 	&\
	% 	\src{t}
	% \\
	\src{t} \bnfdef
		&\
		\src{n} \mid \src{t\op t} \mid \src{\ifztes{t}{t}{t}} \mid \src{\letins{x}{t}{t}} \mid \src{\pair{t,t}} \mid \src{\projone{t}} \mid \src{\projtwo{t}} \mid \sends{t}
	\\
	\src{v} \bnfdef
		&\
		\src{n} \mid \src{\pair{v,v}}
	\qquad\qquad\qquad
	\src{\tau} \bnfdef
		\
		\src{N} \mid \src{\tau\times\tau}
	\\
	\src{\evalctx} \bnfdef
		&\
		\src{\hole{\cdot}} \mid \src{\evalctx\op t} \mid \src{n\op \evalctx} \mid \src{\ifztes{\evalctx}{t}{t}} \mid \src{\letins{x}{\evalctx}{t}} \mid \src{\projone{\evalctx}} \mid \src{\projtwo{\evalctx}} \mid \sends{\evalctx}
\end{align*}

\Sm is a strongly typed language whose type system is unsurprising.\et{skip the rules?}
\begin{center}
	\typerule{Type-\Sm-send}{
		\src{\Gamma}\vdash\src{t}:\src{\tau\times\tau'}
	}{
		\src{\Gamma}\vdash\src{\sends{t}}:\src{N}
	}{t-sm-send}\and
	\typerule{Type-\Sm-n}{}{
		\src{\Gamma}\vdash\src{n}:\src{N}
	}{t-sm-n}\and
	\typerule{Type-\Sm-op}{
		\src{\Gamma}\vdash\src{t}:\src{N}
		\\
		\src{\Gamma}\vdash\src{t'}:\src{N}
	}{
		\src{\Gamma}\vdash\src{t\op t'}:\src{N}
	}{t-sm-op}\and
	\typerule{Type-\Sm-if}{
		\src{\Gamma}\vdash\src{t}:\src{N}
		\\
		\src{\Gamma}\vdash\src{t'}:\src{\tau}
		&
		\src{\Gamma}\vdash\src{t''}:\src{\tau}
	}{
		\src{\Gamma}\vdash\src{\ifztes{t}{t'}{t''}}:\src{\tau}
	}{t-sm-if}\and
	\typerule{Type-\Sm-let}{
		\src{\Gamma}\vdash\src{t}:\src{\tau}
		\\
		\src{\Gamma,x:\tau}\vdash\src{t'}:\src{\tau'}
	}{
		\src{\Gamma}\vdash\src{\letins{x}{t}{t'}}:\src{\tau'}
	}{t-sm-let}\and
	\typerule{Type-\Sm-pair}{
		\src{\Gamma}\vdash\src{t}:\src{\tau}
		\\
		\src{\Gamma}\vdash\src{t'}:\src{\tau'}
	}{
		\src{\Gamma}\vdash\src{\pair{t,t'}}:\src{\tau\times\tau'}
	}{t-sm-pair}\and
	\typerule{Type-\Sm-p1}{
		\src{\Gamma}\vdash\src{t}:\src{\tau\times\tau'}
	}{
		\src{\Gamma}\vdash\src{\projone{t}}:\src{\tau}
	}{t-sm-p1}\and
	\typerule{Type-\Sm-p2}{
		\src{\Gamma}\vdash\src{t}:\src{\tau\times\tau'}
	}{
		\src{\Gamma}\vdash\src{\projtwo{t}}:\src{\tau'}
	}{t-sm-p2}\and
\end{center}

The operational semantics of \Sm is a contextual, small-step, call by value semantics.
Additionally, \Sm has a big-step semantics that produces traces, i.e., queues \src{Q} of messages \src{M} (i.e., pairs) sent over the network.
% We can decouple the sending of the message from the actual operator to show how this scales in a concurrent send, but this is not done here for simplicity.
\begin{align*}
	% \src{\Omega} \bnfdef
	% 	&\
	% 	\src{Q\tr t}
	% \\
	\src{Q} \bnfdef
		&\
		\srce \mid \src{M ; Q}
	% \\
	&
	\src{M} \bnfdef
		&\
		\src{\pair{v,v}}
	% \\
	&
	\src{\alpha} \bnfdef
		&\
		\src{M} \mid \src{\epsilon}
\end{align*}

% The semantics rely on these judgements:
% \begin{align*}
% 	\src{t \sem Q}
% 	&&&
% 	\text{Term \src{t} emits trace \src{Q}.}
% 	\\
% 	\src{t \Xtos{Q} t'}
% 	&&&
% 	\text{Term \src{t} produces trace \src{Q} and becomes \src{t'}.}
% 	\\
% 	\src{t \xtos{\lambda} t'}
% 	&&&
% 	\text{Term \src{t} steps in one step to \src{t'} emitting \src{\lambda}.}
% \end{align*}

\mytoprule{\src{t \xtos{\alpha} t'} }
\begin{center}
	\typerule{Eval-\Sm-Op}{
		\src{n''}=n\op n'
	}{
		\src{n\op n'\xtos{\epsilon} n''}
	}{e-sm-op}\and
	\typerule{Eval-\Sm-Let}{
	}{
		\src{\letins{x}{v}{t} \xtos{\epsilon} t\subs{v}{x}}
	}{e-sm-let}\and
	\typerule{Eval-\Sm-P1}{
	}{
		\src{\projone{\pair{v,v'}} \xtos{\epsilon} v}
	}{e-sm-p1}\and
	\typerule{Eval-\Sm-P2}{
	}{
		\src{\projtwo{\pair{v,v'}} \xtos{\epsilon} v'}
	}{e-sm-p2}\and
	\typerule{Eval-\Sm-If-t}{
	}{
		\src{\iftes{0}{t}{t'} \xtos{\epsilon} t}
	}{e-sm-if-t}\and
	\typerule{Eval-\Sm-If-f}{
		\src{n}>\src{0}
	}{
		\src{\iftes{n}{t}{t'} \xtos{\epsilon} t}
	}{e-sm-if-f}\and
	\typerule{Eval-\Sm-Send}{}{
		\src{\sends{\pair{v,v'}} \xtos{\pair{v,v'}} 0}
	}{e-sm-send}
	% \typerule{Eval-\Sm-Ctx}{
	% 	\src{t\xtos{\lambda} t'}
	% }{
	% 	\src{Q\tr \evalctxs{t} \xtos{\epsilon} \lambda;Q\tr \evalctxs{t'}}
	% }{e-sm-ctx}\and
	% \typerule{Eval-\Sm-Net}{}{
	% 	\src{M;Q\tr t \xtos{M} Q\tr t}
	% }{e-sm-net}
\end{center}
\botrule

\mytoprule{\src{t \Xtos{Q} t'} ~~\vrule~~ \src{t \sem Q}}
\begin{center}
	\typerule{E\Sm-refl}{
	}{
		\src{t} \Xtos{} \src{t}
	}{ev-s-refl}
	\typerule{E\Lt-silent}{
		\src{t}\xtos{\epsilon}\src{t'}
	}{
		\src{t}\Xtos{}\src{t'}
	}{beh-s-silent}
	\typerule{E\Lt-single}{
		\src{t}\xtos{\alpha}\src{t'}
	}{
		\src{t}\Xtos{\alpha}\src{t'}
	}{beh-s-sin}
	\typerule{E\Sm-trans}{
		\src{t}\Xtos{Q}\src{t''}
		&
		\src{t''}\Xtos{Q'}\src{t'}
	}{
		\src{t}\Xtos{Q;Q'}\src{t'}
	}{beh-s-cons}
	\vrule
 %    \typerule{E\Sm-cons}{
	% 	\src{t}\xtos{\lambda}\src{t''}
	% 	&
	% 	\src{t''}\Xtos{Q}\src{t'}
	% }{
	% 	\src{t}\Xtos{\lambda; Q}\src{t'}
	% }{beh-s-cons}
	\typerule{Sem-\Sm}{
		\exists \src{v}\ldotp
		\src{t\Xtos{Q}v }
	}{
		\src{t\sem Q}
	}{sem-s}
\end{center}
\botrule
In \Cref{tr:beh-s-sin} notice that if \src{\alpha} is \src{M} we enqueue that single element, whereas if \src{\alpha} is \src{\epsilon}, we enqueue the empty queue.
We assume that queuing the empty element is ineffective: $Q = \epsilon;Q$.


\subsubsection{\Tm: Target}
\Tm is a statically-typed language with the same types as \Sm, but its primitive for over a network interface only sends \emph{natural numbers}.
Nothing changes regarding terms, values, types and evaluation contexts between \Tm and \Sm.
There is only one typing rule that changes, the one for \sendt{n}, all other ones are as in \Sm.
\Tm has the same dynamic semantics of \Sm, the only changes are to what messages are and to the primitive reduction for \sendt{n}.
\begin{center}
	$\trg{M} \bnfdef\ \trg{n}$
	\and
	\typerule{Type-\Tm-send}{
		\trg{\Gamma}\vdash\trg{t}:\trg{N}
	}{
		\trg{\Gamma}\vdash\trg{\sendt{t}}:\trg{N}
	}{t-tm-send}\and
	\typerule{Eval-\Tm-Send}{}{
		\trg{\sendt{n} \xtot{n} 0}
	}{e-tm-send}\and
\end{center}


\subsubsection{\compm{\cdot}: Compiler from \Sm to \Tm}
The compiler from \Sm to \Tm is defined inductively on the type derivation of a source term, so $\cmpm{\cdot} : \src{\Gamma\vdash t:\tau}\to\trg{t}$.
The only interesting case is when compiling a \src{\sends{t}}, where we use the source type information concerning the message (i.e., a pair) being sent to deconstruct that pair into a sequence of natural numbers, which is what is sent in the target.

The compiler operates on \emph{type derivations} for terms.
Thus, compiling \src{s;s'} would look like the following (using \src{D} as a metavariable to range over derivations).
\begin{align*}
  \compm{
    \AxiomC{\src{D}}
    \UnaryInfC{$\vdash\src{s}$}
    	\AxiomC{\src{D'}}
    	\UnaryInfC{$\vdash\src{s'}$}
    \BinaryInfC{$\vdash\src{s;s'}$}
    \DisplayProof
  } 
  =&\
  \trg{
  	\compm{
  	    \AxiomC{\src{D}}
  	    \UnaryInfC{$\vdash\src{s}$}
  	    \DisplayProof
  	}
    ;
    \compm{
	    \AxiomC{\src{D'}}
	    \UnaryInfC{$\vdash\src{s'}$}
	    \DisplayProof
	}
  }
\end{align*}
However, note that each judgment uniquely identifies which typing rule is being applied and the underlying derivation.
Thus, for compactness, we only write the judgment in the compilation and implicitly apply the related typing rule to obtain the underlying judgments for recursive calls.
\begin{align*}
	\compm{\src{\Gamma\vdash n:N}}
		&\ =
		\trg{n}
	&
	\compm{\src{\Gamma\vdash\projone{t}:\tau}}
		&\ =
		\trg{\projone{\compm{\src{\Gamma\vdash t:\tau\times\tau'}}}}
	\\
	\compm{\src{\Gamma\vdash t\op t' : N}}
		&\ =
		\trg{\compm{\src{\Gamma\vdash t : N}}\op\compm{\src{\Gamma\vdash t' : N}}}
	&
	\compm{\src{\Gamma\vdash\projtwo{t}:\tau'}}
		&\ =
		\trg{\projtwo{\compm{\src{\Gamma\vdash t:\tau\times\tau'}}}}
\end{align*}
\begin{align*}
	\compm{\src{\Gamma\vdash\ifztes{t}{t'}{t''}:\tau}}
		&\ =
		\trg{
			\begin{aligned}[t]
				&
				\ifztet{
					\compm{\src{\Gamma\vdash t:N}}
					% \\
					% &\
				}{
					\compm{\src{\Gamma\vdash t':\tau}}
				}{
					\compm{\src{\Gamma\vdash t'':\tau}}
				}
			\end{aligned}
		}
	\\
	\compm{\src{\Gamma\vdash\letins{x}{t'}{t''}:\tau'}}
		&\ =
		\trg{
			\begin{aligned}[t]
				&
				\letint{
					\trg{x}
				}{
					\compm{\src{\Gamma\vdash t':\tau}}
					% \\
					% &\
				}{
					\compm{\src{\Gamma,x:\tau\vdash t'':\tau'}}
				}
			\end{aligned}
		}
	\\
	\compm{\src{\Gamma\vdash\pair{t,t'}:\tau\times\tau'}}
		&\ =
		\trg{
			\pair{\compm{\src{\Gamma\vdash t:\tau}},\compm{\src{\Gamma\vdash t':\tau'}}}
		}
	\\
	\compm{\src{\Gamma\vdash\sends{t}:N}}
		&\ =
		\trg{
			\letint{
				x
			}{
				\compm{\src{\Gamma\vdash t:\tau\times\tau'}}
			}{ \gensend{x}{\tau\times\tau'} }
		}
\end{align*}

The \gensend{\cdot}{\cdot} function takes a term and its source-level type and returns a list of target send instructions that send each element of the term.
\begin{align*}
	\gensend{t}{\tau} =
		\begin{cases}
			\trg{\sendt{t}} & \ift \src{\tau} = \src{N}
			\\
			\trg{
				% \sendt{\falset};
				\gensend{\projone{t}}{\tau'};
				\gensend{\projtwo{t}}{\tau''}
				% ;\sendt{\truet}
			}
			& \ift \src{\tau} = \src{\tau'\times\tau''}
		\end{cases}
\end{align*}



\subsubsection{Relating Traces}
We start with the trivial relation between numbers: $\src{n}\sim\trg{n}$, i.e., numbers are related when they are the same number.
% \et{this trivial relation is not needed, since we're only relating traces, fully-covered with the defs below} MARCO: actually it's needed, i forgot to use it, thanks!

We cannot build a relation between single messages since a single source message gets related to multiple target ones.
However we can build a relation between a source message and a target queue of messages: $\src{M}\sim\trg{Q}$, defined inductively on the structure of \src{M}.
\begin{center}
	\typerule{Trace-Rel-N-N}{
		\src{n}\sim\trg{n}
		&
		\src{n'}\sim\trg{n'}
	}{
		\src{\pair{n,n'}} \sim\trg{n;n'}
	}{tr-rel-n}
	\typerule{Trace-Rel-N-M}{
		\src{M}\sim\src{Q}
	}{
		\src{\pair{n,M}}\sim\trg{n;Q}
	}{tr-rel-n-m}
	\typerule{Trace-Rel-M-N}{
		\src{M}\sim\src{Q}
	}{
		\src{\pair{M,n}} \sim\trg{Q;n}
	}{tr-rel-m-n}
	\typerule{Trace-Rel-M-M}{
		\src{M}\sim\src{Q}
		&
		\src{M'}\sim\src{Q'}
	}{
		\src{\pair{M,M'}} \sim\trg{Q;Q'}
	}{tr-rel-m-m}
\end{center}
A pair of naturals is related to the two messages that send each element of the pair (\Cref{tr:tr-rel-n}).
Otherwise, if we split a pair into sub-pairs, we request all such sub-pairs to be related (\Cref{tr:tr-rel-n-m,tr:tr-rel-m-n,tr:tr-rel-m-m}).

With this we can define when a source trace is related to a target one: $\src{Q}\sim\trg{Q}$.
\begin{center}
	\typerule{Trace-Rel-Single}{
		\src{Q}\sim\trg{Q}
		&
		\src{M}\sim\trg{Q'}
	}{
		\src{Q;M}\sim \trg{Q;Q'}
	}{tr-rel-full}
	\typerule{Trace-Rel-Empty}{
	}{
		\srce\sim \trge
	}{tr-rel-empty}
\end{center}
Trivially, queues are related when they are both empty (\Cref{tr:tr-rel-empty}).
Alternatively, given related queues, we can concatenate a source message and a second target queue only if they are related (\Cref{tr:tr-rel-full}).



\subsubsection{Proof of Compiler Correctness}
To prove that the compiler is correct (\Cref{thm:inst-marco-cc}) we need an auxiliary result (\Cref{thm:inst-marco-gensend}) telling us that the way we break down a source send into multiple target ones is correct.
For brevity, proofs are omitted \MP{ ref to coq or appendix}\et{+1}
\begin{lemma}[\gensend{\cdot}{\cdot} is correct]\label{thm:inst-marco-gensend}
	$\ift
	\trg{\gensend{\compm{\src{\Gamma\vdash v : \tau\times\tau'}}}{\tau\times\tau'} \Xtot{Q} 0}
	\thent
	\src{v}\sim\trg{Q}$
\end{lemma}


\begin{theorem}[\compm{\cdot} is correct]\label{thm:inst-marco-cc}
$\vdash\compm{\cdot}:\tildePF{\traceP}$
\end{theorem}
\et{the statement uses a non-introduced syntax $\vdash \_ :\tildePF{\traceP}$}
\MP{ yes: i expect this syntax will be defined above. It's syntax that is used in order to state that a compiler upholds a certain criterion}




\subsubsection{Possible Extensions: Inputs}

\mbox{}\et{not sure what the point of this subsection is. There does not seem to be anything to put forth as such}
\MP{
	at some point we discussed whether we should add inputs,
	these are my thoughts on why adding inputs is not necessary and does not lead to necessarily new insights.
	I expect this will be moved to the appendix.
}

This section considers the addition of another source of trace events to the languages: inputs.
We have different ways to model inputs, though we argue that none of them add insights beyond what already developed.
\begin{enumerate}
	\item \Sm inputs \src{N} and \Tm inputs \trg{N}.

	In this case the source program must already contain the code to ``compose'' the inputs into larger data structures (i.e., into larger pairs).
	Compiling such a program adds nothing to what already provided.

	\item \Sm inputs \src{\tau\times\tau} and \Tm inputs \trg{N};

	In this case the source program handles inputs as pairs while the target handles them as single naturals.
	Necessarily, the compiled program must therefore contain additional instructions to compose a pair such as the source one starting from individual naturals.
	This is the dual case of the compilation of output, so it adds no particular insight.
	Instead of having \gensends{\cdot}, we would need another function that \emph{relying on the type information} (which is available through compilation), builds a target pair that behaves like the source level one.

	\item \Sm inputs \src{N} and \Tm inputs \trg{\tau\times\tau};

	In this case the target seems more expressive than the source
	How can we compile a ``\src{read}~\src{n}'' into a ``\trg{read}~\trg{\pair{n',n''}}''? \et{just \trg{read}~\trg{\pair{n',0}}? (by analogy with the out case below)} 

	On one hand, this seems orthogonal to also having outputs, it's more of an issue of how to treat inputs.
	In fact, if we did the opposite of the above, so output \src{N} in \Sm but output \trg{\tau\times\tau} in \Tm,
	we would compile ``\src{out~n}'' into ``\trg{out~\pair{\compm{n},0}}''.

	More generally, thus, the issue is how to deal with inputs.
	Typically, the code after the read will have to case it in case we need to react to specific inputs.
	That code will also be present in the compiled code (it comes from the source), but the issue would be: what element of the pair should we pick in the target?
	If the target pair models a multiple input port with different quality of value, it may be worth to consider a backtracking approach, i.e., we compute with the first projection and if that fails, we backtrack and continue with the second.
	However, this seems vastly orthogonal to the issue of relating traces, it's more of a system design issue.

	Thus, this option is also not leading to any particularly interesting case (w.r.t. cross-trace relations at least).

	\item \Sm inputs \src{\tau\times\tau} and \Tm inputs \trg{\tau\times\tau};

	In this case there is no abstraction gap, so adding inputs does not lead to any particularly interesting case.
\end{enumerate}


==> mappings.tex <==
% !TeX root = main.tex

As explained in \autoref{sec:intro}, trace-relating compiler correctness
\cctilde, by itself, lacks a crisp description of which trace properties
are preserved by compilation.
%
Since even the syntax of traces can differ between source and target, one can
either look at trace properties of the source (but then one needs to interpret
them in the target), or at trace properties of the target (but then one needs to
interpret them in the source).
%
\ch{Text that can't stay without improvements:
The first interpretation could answer the following question: what guarantees
does one obtain when compiling a verified C program that does not encounter an
undefined behavior to machine code (\autoref{sec:example-undef})?
%
The second interpretation could tell us what condition in the source prevents a
compiled program from failing with an out of memory violation
(\autoref{sec:example-resources}). \ca{reading \autoref{sec:example-resources} again 
this statement sounds a bit odd. In that subsection indeed we show (and this is given 
by the fact that we do not have a lower bound on the resource exhaustion e.g. you cannot
finish your resources before $k$ steps) that if we want a non empty source interpretation of
a property $\piT{\pi}$, then if $\piT{\pi}$ contains a trace $\tT{t}$ then it must
contain all traces of the form $m\cdot \ii{Resource\_Limit\_Hit}$ with
$m \leq \tT{t}$ }\ch{Both examples sound strange to me. I don't know what the
answers are to be honest. Do you? Section 3.2 says this: ``any property that
prevents resource exhaustion cannot be proved using source-level reasoning'' --
so the $\sigma$ is trivial!?}}
%
% CH: Just reexplaining stuff from the intro in a very poor way
% \begin{enumerate}
% \item\label{pt:1} the strongest target property $\piT{\pi}$, such that
%   $\cmp{W} ~\satT~ \piT{\pi}$ holds for any $\src{W}$ for which we can show that
%   $\src{W} ~\satS~ \src{\pi_S}$ (\EG by formal verification)
% %
% \item\label{pt:2} the weakest source property $\src{\pi_S}$ whose satisfaction
%   suffices to $\cmp{W} ~\satT~ \piT{\pi}$, for a fixed $\piT{\pi}$, target
%   property of particular interest.
% \end{enumerate}
% $\ii{CC}^{\sim}$ does not provide a direct answer to the above questions. 
% \\
% \MP{ what is TCtilde? it's a new acronym. Also, i don't think telling what TCtilde does not do is helpful unless we get to know what TCtilde also does... which seems to come way later } 
% \ca{changed to $\ii{CC}^{\sim}$}
% Similarly to $\pf{\traceP}$,\ch{not introduced yet, maybe in intro?}\et{I suggest a new 2.1 section on background}
% the statement of $\ii{CC}$ is ``property-free''. \ca{TODO: check if this term is introduced before}
% %
% When trying to bring properties into the picture,\ch{for TC-TP this
%   story is simpler, as currently explained in abstract and probably in
%   the intro}
% %
% two important questions arise:
% To answer these questions, we need in general an interpretation of source properties in the target and viceversa.
%
Formally, these two interpretations can be seen as two property mappings: 
\begin{align*}
  \tau :&\ \propS \to \propT 
  &
  \sigma :&\ \propT \to \propS
\end{align*}
%
% \et{notation: use $\mathcal{P}(\mathit{Trace}_{S})$ instead of $\propS$?}
% \ch{I like the current notation more}
% 
%
% \et{give some intuition before going to the GC requirement}\ch{+1 this gets
%   super technical too quickly ... there is currently very little motivation,
%   beyond Carmine \MP{and marco :) (though i agree on the need for intuition)} finding Galois connections very cool.}
%
For an arbitrary source program $\src{W}$,
$\tau$ interprets a source property $\piS{\pi}$
as the \emph{target guarantee} for $\cmp{W}$.
% addressing the shortcomings listed in \Cref{pt:1} above).
%
Dually, $\sigma$ defines a \emph{source obligation} sufficient for the
satisfaction of a target property $\piT{\pi}$ after compilation.
%
 % (addressing the shortcomings of \Cref{pt:2}).
To be coherent with this informal interpretation, extra conditions on
$\tau$ and $\sigma$ seem natural (and as we will see in
\autoref{sec:mapping-preservation}):
%
\begin{itemize}[nosep]
\item Given $\piS{\pi}$, the source obligation to get the
  guarantee $\tau(\piS{\pi})$, should not be harder than $\piS{\pi}$
  itself, \IE~$\sigma(\tau(\piS{\pi})) \supseteq \piS{\pi}$.
%
%  First, the source property obtained by applying $\sigma$ to the guarantee
%   obtained by interpreting $\piS{\pi}$ in the target (via $\tau$)
% % \MP{there's a sigma too many or you meant something else? Also below. If it's interpreted in the target it should only be tau(pi)}
% % \et{no, it's correct, it's the source obligation (sigma) of the target interpretation (tau) -- I added some text to be clearer}
% should be weaker than
% $\piS{\pi}$ itself, \IE~$\sigma(\tau(\piS{\pi})) \supseteq \piS{\pi}$.
\item Dually, for $\piT{\pi}$, the target interpretation of
  the source obligation $\sigma(\piT{\pi})$ should actually guarantee
  that $\piT{\pi}$ holds,
  \IE~$\tau(\sigma(\piT{\pi})) \subseteq \piT{\pi}$
%
%  Dually, the target property obtained via $\tau$ from the source obligation
%   (via $\sigma$) for a target property $\piT{\pi}$
% should actually ensure that $\piT{\pi}$ holds, \IE~$\tau(\sigma(\piT{\pi})) \subseteq \piT{\pi}$. 
%
\end{itemize}
These two conditions on $\tau$ and $\sigma$ are satisfied 
% exactly\ch{right?} \ca{you also need continuity of the two mappings }
when the two maps form a {\em Galois connection} between the posets of source
and target properties ordered by inclusion.
%
Let us first recall the definition and the characteristic property of Galois connections~\cite{CousotCousot77-1, Melton:1986}.
%
\begin{definition}[Galois connection] Let $(X, \preceq)$ %\ch{This clashes with prefix notation! Can we change here?}
and $(Y, \sqsubseteq)$ be two posets.
  A pair of maps, $\alpha: X \to Y$, $\gamma: Y \to X$ is a Galois connection \ii{iff}
  it satisfies the following \emph{adjunction law}:
                      $\forall x \in X. ~ \forall y \in Y. ~ \alpha(x) \sqsubseteq y \iff x \preceq \gamma(y)$.
                   % \begin{equation*} 
                   % \end{equation*}
$\alpha$ is referred to as the lower adjoint and $\gamma$ as the upper adjoint.
\end{definition}
%
We will often write
$\alpha: (X, \preceq) \leftrightarrows (Y, \sqsubseteq) :\gamma$ to
denote a Galois connection, or simply
$\alpha: X \leftrightarrows Y :\gamma$,
% when $X$ and $Y$ are powersets
% with inclusion
or even $\alpha \leftrightarrows \gamma$ when the
involved posets are clear from context.
%
%
\begin{lemma}[Characteristic property of Galois connections] \label{lem:chG}
  If $\alpha{:} (X, \preceq) \leftrightarrows {(Y, \sqsubseteq) {:}\gamma}$ is a Galois connection, then $\alpha, \gamma$ are monotone and
  they satisfy these properties:
  \begin{align*}
   i)& \quad \forall x \in X.  ~ x \preceq \gamma(\alpha (x)) 
   % \\
   &
   ii)& \quad \forall y \in Y. ~ \alpha(\gamma (y)) \sqsubseteq y
  \end{align*}
%
If $X,Y$ are complete lattices, then $\alpha$ is continuous,
\IE~$\forall F \subseteq X.  ~\alpha(\bigsqcup F) = \bigsqcup \alpha(F)$.
\end{lemma}
%
These properties coincide with the
conditions on property mappings introduced above, taking $X$ to be source
properties, $Y$ to be target properties, $\alpha$ to be $\tau$,
$\gamma$ to be and $\sigma$, and the order to be set inclusion, \IE
$\sigma(\tau(\piS{\pi})) \supseteq \piS{\pi}$ and
$\tau(\sigma(\piT{\pi})) \subseteq \piT{\pi}$.%

\ca{two reviewers complained about the clarity of the following}
Perhaps surprisingly, the property mapping to the target ($\tau$) corresponds to
the abstraction function $\alpha$, while the property mapping to the source
($\sigma$) corresponds to the concretization function $\gamma$.
%
The explanation is that the definition of trace properties $\prop$ is
contravariant in $\text{Trace}$, so while traces get more concrete when moving
to the target, trace properties get, well, more abstract.
%
%
\subsection{Revisiting Trace Property Preservation}
\label{sec:mapping-preservation}
% \et{made that a new subsection} \et{btw, here's an example where mapping subsections to files is awkward, because one might want to evolve the structure more flexibly}
%
We can now generalize trace property preservation ($\traceP$), relying
on an interpretation of source properties in the target and target properties in the source. 
%
\begin{definition}[\tpsigma and \tptau] \label{defn:TP}
 Given two property mappings, $\tau : \propS \rightarrow 2^\trg{Trace_T}$ and
  $\sigma : \propT \rightarrow\propS$,
%
%\MP{ defined less than a page ago}
% \ca{No, it's not $\tilde{\tau}$, these definitions are for abritrary mappings, }
%
for a compilation chain $\cmp{\cdot}$ we define:
%
%   \begin{align*}
%     \tptau: \quad
%     \forall \piS{\pi} \in\propS. ~\forall \src{W}.~
%     &
%       (\forall \tS{s} \ldotp \src{W \sem} \tS{s} \Rightarrow \tS{s}\in\src{\pi_S})
%       \Rightarrow
%       (\forall ~\tT{t} \ldotp \cmp{W} \trg{\sem} \tT{t} \Rightarrow \tT{t}\in\tau(\src{\pi_S}))
%     \\
%     \tpsigma: \quad
%     \forall \piT{\pi} \in \propT.~\forall\src{W}.~
%     &
%       (\forall \tS{s} \ldotp \src{W \sem} \tS{s} \Rightarrow \tS{s}\in \sigma(\piT{\pi}))
%       \Rightarrow
%       (\forall \tT{t} \ldotp \cmp{W} \trg{\sem} \tT{t} \Rightarrow \tT{t}\in\piT{\pi})
% \end{align*}
%
{\small
\[
    \tptau \equiv
    \forall \piS{\pi}. ~\forall \src{W}. ~ \src{W} ~\satS~ \piS{\pi} \Rightarrow 
                                                      \cmp{W} ~\satT~ \tau(\piS{\pi}) 
\quad
    \tpsigma \equiv
    \forall \piT{\pi}. ~\forall\src{W}.~ \src{W} ~\satS~ \sigma(\piT{\pi}) \Rightarrow 
                                                   \cmp{W} ~\satT~ \piT{\pi}
\]
}
\end{definition}
%\et{with notation suggested, this would read simply as: 
%$\forall \piS{\pi}, \src{W}.\; \src{W} \vDash \piS{\pi} \Rightarrow \cmp{W} \vDash \tau(\piS{\pi}) $}
%
% \bigskip
%
%
% The map $\tau$ describes the \emph{target assurance}
% %\ca{or taget guarantee?}
% for $\cmp{W}$, while $\sigma$ defines the \emph{source obligation}
% %\emph{source proof obligation} \et{what about simply "source obligation" (symmetry with "target assurance")}
% for the satisfaction of a target property.\footnote{The Greek letters $\tau$
%   and $\sigma$ have been chosen to suggest their codomains,
%   \emph{``target''} and \emph{``source''} respectively. }
%
% For example, $\tau$ may tell us what is ensured in the target language
% when the source property \emph{``The program does not encounter an
%   undefined behavior''} (\Cref{sec:example-undef}) is
% satisfied. Dually, $\sigma$ imposes a condition that guarantees the
% satisfaction of a given target property,
% even if more precise observations are possible in the target (\Cref{sec:example-noninterference}). 
%
%
% \et{better structure: first introduce $\tau$ and $\sigma$, and their intuitions. Then the GC. Then, and only then, introduce the TPs and the equivalences.}
% \ca{I am following this advice}
% \et{good!}
%
% To stay coherent with these intents,
% the proof obligation for a source property, interpreted in the target \et{ie. $\sigma(\tau(\piS{\pi}))$}, should not require a bigger effort than a direct proof of the same property \et{$\piS{\pi}$},
% i.e. $\sigma(\tau(\piS{\pi})) \supseteq \piS{\pi}$. Similarly, the source proof obligation of a target property, should be interpreted in the
% target as a sufficient condition for the original property, i.e. $\tau(\sigma(\piT{\pi})) \subseteq \piT{\pi}$.\et{ie: "the target assurance of the source obligation should be sufficient"}
%
%
%
% \ch{We are still badly missing intuition why a Galois connection is a
%   reasonable thing to require/expect here. Simply making the proof
%   below work does not count as intuition!}\ch{I'm starting to revert
%     my opinion on this. It could be that wanting Theorem 2.4 is an okay
%     way to motivate the Galois connection.}
% \et{the discussion in 2.1 (with the bullets) motivates the equations intuitively}
%
%
% The above mentioned conditions also provide the equivalence of \critdiff{\tp}{\tau} and \critdiff{\tp}{\sigma} (\Cref{thm:galois}).
% They can be formalized with the notion of a \emph{Galois connection} \cite{CousotCousot77-1, Melton:1986},
% that we briefly recall together with some of their properties.
%
% \bigskip
%
By uniqueness of adjoints \cite{Melton:1986}, given a $\tau$, there
exists at most one $\sigma$ such that the two form a Galois connection
(and vice versa).  Here, this means that, in compiler design, the
source obligations, $\sigma$, are uniquely defined by the target
guarantees $\tau$ and viceversa.
%
This intuition is formally captured by the following theorem that show
the equivalence of $\tptau$ and $\tpsigma$, everytime $\tau$ and
$\sigma$ form a Galois connection.
%
\begin{theorem}[\tptau and \tpsigma coincide \coqhref{Def.v}]
\label{thm:galois}
 Let  $\tau :  2^\src{Trace_S} \rightleftarrows \propT : \sigma$
 be a Galois connection, 
%\et{that notation *is* for a GC, so not correct to state "If ... is a GC" -- use "Let ... be a GC, then..."}
 with $\tau$ and $\sigma$ the lower and upper adjoints (resp.). 
 Then
 $ \tptau \iff \tpsigma $.

\end{theorem} 
\ifsooner
\ch{Does the other direction of the theorem above hold?  Can we obtain
  that $\tau$ and $\sigma $ form a Galois connection from a proof that
  $ \tptau \iff \tpsigma$?}
\fi
% \rb{So is this going both directions? Clarify with above. This is a bit
%     confusing to read, for me.}
% \ca{tried to clarify}


==> old-sc-diagram.tex <==

Due to spaces constraints, %\ca{time and lower-back pain :P \MP{:D}} 
we do not list all the definitions for the criteria for all possible subclasses.
Instead, we provide an illustrative diagram of the criteria from \cite{AbateBGHPT19} that are brought to the trace-relating setting (\autoref{fig:diagram-preserve-props-sec})
and describe a way to navigate it.
The diagram indicates with a \CoqSymbol the trinities whose equivalences have been proven in Coq.
The interested reader will find omitted definitions in the anonymous supplementary materials. 
% \MP{file!}\MP{ i really think that if you have time, you should write at least the tilde for all of these and put them in an appendix. i bet you can do it in 30 minutes :)}
\input{diagram-prop-pres-comp-security}
For a given trace relation $\sim$, the diagram orders the generalized criteria according to their relative strength (higher is stronger); if a trinity implies another, then the former is stronger.
Moreover, it shows that for all of them a trinitarian view is possible. 
Every point in the diagram has one of the two following shapes: \formatCompilers{R~\_~P^{(\cdot)}} or \formatCompilers{R~\_~C^{\sim}}.
In either case the common hole $(\_)$ is filled with an acronym of some class of (hyper)properties or relational (hyper)properties. 
We adopt the acronyms of \citet{AbateBGHPT19}, so H means ``hyperproperties'', SCH means ``subset-closed hyperproperties'', HS means ``hypersafety'', T means ``trace properties'' and S means ``safety properties''.
% As before, we use the convention that the property-ful criterion ends with a $C$ and it is on top in the trinities.
% The property-free criteria derived from $\sigma$ and $\tau$ are always respectively left and right and their name ends with $P$.
The second hole of  \formatCompilers{R~\_~P^{(\cdot)}} is filled with an operator that can be one of $\tilde{\tau}$ and $\tilde{\sigma}$.
In certain cases, as explained in \autoref{sec:safety-preservation} for compiler correctness, this operator is composed with an upper closed operator
that ensures the final image will be in the considered class of (relational)(hyper)properties.
As seen before, composing with $\ii{Safe}$ (\IE $\ii{Safe} \circ \tilde{\tau}(\piS{\pi})$) we have a safety property for arbitrary $\piS{\pi}$.    
%
% As previously mentioned, this closure is needed because certain property-free criteria do not follow from their property-full one but from a stronger one that is closed under a certain class of properties.
% This is the case for \critdiff{RSC}{\tilde{\tau}}, which instead is derived from closing \ii{RTC} with safety properties, \IE \critdiff{RTC}{\ii{Safe} \circ \tilde{\tau}} (as was happening in \autoref{thm:trini-safe}). 
% \ca{this last sentence is not precise, the property full you are mentioning are nor stronger nor weaker, e.g. for RSCtilde the 
%     property full with tau says that you can consider arbitrary trace properties in the source, but in the target you 
%     get a guarantee only on the safety closure of tau (that is larger than tau, hence a weaker guarantee) }

To facilitate reading the diagram, we color the three points that distinct properties (\tcol) from hyperproperties (\sccol) and relational properties (\trtcol). 
Notice that when a closure is needed, e.g. $\ii{Safe}$, a colored box that highlights the quantification on a lager class than the one suggested by the other acronyms in the trinity,
e.g. for \rsptautilde the $\tcol~$ box remarks the quantification on all source trace properties (not only safety ones).
%the trinity from which the stronger criterion is borrowed in order to realize that a criterion is not derived from the current trinity but from a different one (with the same background color).
%Specifically, the trace-based trinity is \tcol, the subset-closed hyperproperty one is \sccol, and 2-relational trace properties are \trtcol.
% \MP{
%   sentence below is .. ?
% }
% The $R~\_~P^{(\cdot)}$ criteria are compared with $R~\_~C^{\sim}$ that generalizes the property-free statements from \cite{AbateBGHPT19} to the trace-relating setting.

==> rel_to_maps.tex <==
% !TeX root = main.tex

We now investigate the relation between $\cctilde$ and
\tptau and \tpsigma.
%
We show that, starting from a given trace relation
$\sim$, it is always possible to define two property mappings $\tilde{\tau}$,
$\tilde{\sigma}$ so that the three criteria are all equivalent.
% (\Cref{thm:allequiv}).
%
Dually, \autoref{sec:trinity2} will show that, given a Galois connection
$\tau \rightleftarrows \sigma$, it is possible to define a relation that
ensures the equivalence. %(\Cref{thm:rel}).
%% \MP{
%%   missing leading text
%% }

% \ch{This is good stuff, something that could guide the structure of this section:}

% CH: this is now in the section outline
% So far we discussed some generalization of trace-based criteria
% for compiler correctness. We showed that it is possible to start either from the property-free
% characterization $\pf{\traceP}$ and a relation between source and target
% traces (\Cref{defn:tracepreservation}), or from $\traceP$ and an interpretation
% of properties of one language into the other (\Cref{defn:TP}).
% %
%
\begin{definition}[Induced property mappings]
\label{defn:ttautsigma}
  For an arbitrary trace relation
  $\sim \,\subseteq \src{Trace_S} \times \trg{Trace_T}$, we define its {\em
    induced property mappings} $\tilde{\tau}$ and $\tilde{\sigma}$ as
  in \autoref{sec:intro}:
  \begin{align*}
    \tilde{\tau}   & = \lambda ~\piS{\pi}. ~ \myset{\tT{t}}{\exists \tS{s} \ldotp \tS{s} \sim \tT{t} \wedge \tS{s} \in \piS{\pi}} 
    % \\
    &
    \tilde{\sigma} & = \lambda ~\piT{\pi}. ~ \myset{\tS{s}}{\forall \tT{t} \ldotp \tS{s} \sim \tT{t} \Rightarrow \tT{t} \in \piT{\pi}}
  \end{align*}
  % \MP{ the notation "tau with the hat" is not explained}
%
% \ch{now these mappings were already introduced in the intro}

\end{definition}
%
These induced property mappings indeed form a Galois connection.% \ch{Not sure why $\tilde{\sigma}_{\ii{naive}}$ is still relevant. For me that
% was just a wrong definition, why would we explain it in the paper?}%
% \footnote{The reader might wonder whether the universal quantification in the definition of $\tilde{\sigma}$ is necessary. For instance, consider 
% $\tilde{\sigma}' = \lambda ~\piT{\pi}. ~ \myset{ \tS{s} }{ \exists \tT{t} \in \piT{\pi}. ~ \tS{s} \sim \tT{t} }$. 
% While intuitively sensible, this definition does not always correspond to the upper adjoint of $\tilde{\tau}$.
% It is however the case that $\tilde{\sigma}'$ and $\tilde{\sigma}$ coincide
% if and only if $\sim$ is a total function from source traces to target traces (\CoqSymbol Theorem $~\sigma$\_$\sigma$\_fwd in NonRobustTraceCriterion.v )} 
% CH: no, not really wondering

\begin{theorem}[Induced adjunction \coqhref{Galois.v}] \label{thm:adjoint}
  $\tilde{\tau} \leftrightarrows \tilde{\sigma}$ is a Galois connection between the sets of trace properties of source and target traces ordered by set inclusion.
\end{theorem}




We denote by \tptautilde, \tpsigmatilde the criteria in \Cref{defn:TP} for $\tilde{\tau}$ and $\tilde{\sigma}$ respectively.
\Cref{thm:allequiv} below states the equivalence of $\tptautilde$, $\cctilde$, and $\tpsigmatilde$:
%
%
\begin{theorem}[$\tptautilde$, $\cctilde$, $\tpsigmatilde$ coincide \coqhref{TraceCriterion.v}]
\label{thm:allequiv}
  For any trace relation $\sim$ and induced property mappings $\tilde{\tau}$ and $\tilde{\sigma}$ (\Cref{defn:ttautsigma}), we have:
  \(\tptautilde \iff \cctilde \iff \tpsigmatilde\).
\end{theorem}
It follows that, for a $\cctilde$ compiler,
$\tilde{\sigma}$ provides the source proof obligation \emph{ensuring} a certain target property holds, and
$\tilde{\tau}$ provides the target \emph{guarantee} of a compiled program every time a property holds for the source program.
%
% As the concrete instances of \autoref{sec:instances} will show, in some specific
% settings t
Sometimes the lifted properties may be trivial: the target guarantee can be
true, and the source obligation can be false.

% \et{discuss here the fact that the lifted properties may simply be impossible to
%   satisfy (there's some discussion of that at the end of 4.1, but it's a bit
%   late)?}\ch{good point; maybe the instances in 3 should explain?}

%
%\ca{TODO: give a look to https://ncatlab.org/nlab/show/Galois+connection#InducedFromARelation }%
%
%


==> relating_src_trg_traces.tex <==
% !TeX root = main.tex
\ch{Need better motivation here, wasn't convinced by next paragraph}

It is often the case that source and target observables, and hence their traces,
can be related. The easiest scenarios one can imagine are those in which traces of a language are a subset
of the other (\Cref{sec:example-undef}), or traces of source language abstract from
some physical restriction, that is instead imposed by target constraints (\Cref{sec:example-resources}, \Cref{sec:example-noninterference}).
% In this last case, a \emph{reasonable}\et{??} compiler should ensure that an execution of a
% compiled program can be simulated by the original program in the source,
% at forgetting, at most, about the target restrictions.\ch{Didn't get
%   the end of this}
%
We propose the following generalization of $\pf{\traceP}$, for an arbitrary \emph{trace relation}, $\sim \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$.
%

\et{terminology to introduce: "trace relation", "trace property mapping"}
\ca{TODO: expand the definition on TC and say \Cref{defn:tracepreservation} is a generalization of the expanded TC}

\begin{definition}[\tildePF{\traceP}] \label{defn:tracepreservation}
Given a trace relation $\sim \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$, we define
\begin{align*}
  \tildePF{\traceP}: \quad\ \forall\src{W}. \forall \tT{t}.~ \wtmkt{W}{t}
         \Rightarrow \mathrel{\exists\tS{s} \sim \tT{t}} \ldotp \wsmkt{W}{s}
\end{align*}
%
\end{definition}

\ch{To explain:
  This is a generalization of the CompCert compiler correctness definition,
  where they use a very specific relation between traces,
  while we allow for any relation.
%
Could potentially use undefined behavior as a running example.}

In order to trust a $\tildePF{\traceP}$ compilation chain, a user should understand, first how source and target traces are related 
by $\sim \,$ and then how this can impact the preservation of semantics properties of programs.
A trivial relation, such as the one relating all source to all target
traces, would make any compiler $\tildePF{\traceP}$, in particular compilers providing no 
guarantee on the preservation of properties.
%
Less trivial relation can still have the same consequences. 

\ca{I gave a name to this relation as we will show later what are the target guarantees for it}
\begin{definition}[Cheating relation] 

We call \emph{cheating} relation for a fixed compilation chain $\downarrow$ the following
trace relation $\sim \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$

  \begin{equation*}
   \tS{s} \sim \tT{t} \iff \exists \src{W}. ~\src{W \sem} \tS{s} \wedge \cmp{W} \trg{\sem} \tT{t}
  \end{equation*}
  
\end{definition}

Assume that every program can emit at least one trace, then an arbitrary compiler $\downarrow$ is 
$\tildePF{\traceP}$ for its cheating relation (\CoqSymbol Theorem cmp\_is\_rel\_TC in Relation4Correctness.v).
We are going to show in \Cref{sec:rel-to-maps} that no guarantee is given on a program compiled by $\downarrow$,
proven to be $\tildePF{\traceP}$ w.r.t its cheating relation.  \ca{TODO: Prove it in Coq}


\et{describe the formalisms intuitively in English (especially important at the beginning of the paper to help the reader)}

\et{is there anything less trivial to say here?}


==> rob-diff-acts.tex <==


\rb{Now I have to clean and mostly remove the old text, relocating some bits to
the discussion. Possibly comment that the proof technique is fairly modular and
extends easily to other relations, as per my (somewhat limited) experience.
Back-translations are not required for these simple languages, but become
necessary in some scenarios. (Say something about (target-only) inputs?
Compartment models?)}

The robust compilation scenario requires us to make explicit the notions of
program and context. \rb{...} It is often useful to resort to a notion of
mutually isolated \emph{compartments}---in the simplest case, a program
compartment and a context compartment---which are allowed to interact solely
through the correct invocation of procedures exposed the \emph{interfaces} of
each component. Commonly, the act of transferring control between components,
i.e., cross-interface calls and returns, will be part of the observable events.

\rb{A very simple extension that may exhibit some of the concepts below could be
  adding \emph{environment variables} to the context, but simply lookups offer
  little chance of generating target-only events.}

In order to prove that a compilation chain robustly preserves a given class of
properties, we will rely on common back-translation techniques \et{cites}. The cornerstone
of such proofs is the construction of source contexts whose behaviors are
related to their associated target contexts (as well as the programs before and
after compilation). This technique may impose restrictions on the source
language based on the target language. For example, if the target language has
mutable state or non-observable inputs, then at the source level calling the same
function with the same inputs may result in different outputs. In order to
obtain a backtranslation of a target context (ab)using such features, the source
language needs to emulate a notion of state, which would be cumbersome \et{meaning?} in a
purely functional setting.
\MP{
  i'm not sure this is at all doable, so i would not claim this
}
%
\rb{Is there any sane way to do this without modifying the source? Even an
  encoding of state using monads seems to need some changes, even if they are
  minor.}

\rb{Normally, an imperative target language will impose some form of
  compartmentalization to isolate the program from direct attacks, for the sake
  of sanity.}

%Irrespective of any other source and target language choices, ...

Consider the source language of simple (functional) expressions.
%
\rb{Describe this ``simplex'' language, or more likely reference to its
  description above.}
%
Let us extend this source language with named functions. For simplicity, suppose
functions have arity exactly one (instead of an arbitrary natural number) \et{i.e. "functions are unary"},
direct or indirect recursive calls are not allowed, and function bodies are simple
expressions extended with bound parameters and function calls.
%
\rb{Illustrate.}
%
\rb{Even simpler variations seem possible. Functions could be replaced by
  non-parametric ``let'' bindings whose bodies are simple expressions. Contexts
  could be simple expressions with a hole into which the a program (another
  simple expression) is plugged. Functions could be first-class constructs
  instead of top-level ones. There are some interactions among these choices,
  but none seem to add or subtract too much from the already simple setting.}
%
Programs and contexts are both partial programs, defined as sets of functions
with unique names satisfying the above restrictions and, optionally, a simple
expression to be evaluated in this scope. Two partial programs can be linked
when they define disjoint sets of function names and at most one defines a
``main'' expression. A program can be executed if all the functions it relies on
are defined and a top-level expression to execute exists.
%
\rb{Some of these ideas need to be made more precise, of course, this is but an
  intuitive approximation.}

\begin{align*}
  e   ::= & n \in \mathbb{N} | e + e | e * e | \text{if}\ e <= e\ \text{then}\ e\ \text{else}\ e \\
  e_f ::= & e | id_{arg} | f e_f \\
  f   ::= & \text{fun}\ id_{fun} id_{arg} = e_f
\end{align*}

\MP{
  given that the formal parameter is only mentioned in ef, and that e does not include ef, functions that use the formal parameter are ONLY identity functions, and all other functions are CONSTANT.
  what is going on here?
}

The first target language we consider is a small extension of the source
language, to which we add the ability to emit an output followed by the
evaluation of another expression.
%
\rb{Again, there are several variations, mostly interesting in the presence of
  ``let'' bindings, otherwise clunky.}
%
The evaluation of this new instruction produces a new, observable event, which
was not present in the source. The semantics of the target language remains
unaltered from that of source language otherwise. The source semantics for whole
programs produces a singleton traces whose sole event contains the result of
evaluating the ``main'' expression.
%
\rb{Saying ``for whole languages'' is not entirely accurate.}

\rb{Describe syntax extension here.}

First, for this pair of languages, consider a semantics whose shared core does
not produce observable events when control is transferred between program and
context. In this case, the relation between source and target traces is rather
simple, though not as informative as it could be if we had information about
control transfers:

\begin{equation*}
  \textit{Result}(n) \sim \textit{Out}_t(n_1) \cdot \ldots \cdot \textit{Out}_t(n_k) \cdot \textit{Result}(n), k \in \mathbb{N}
\end{equation*}

Thus, a source trace that reports a result $n$ is related to all target traces
that report the same result, prefixed by a finite number of target-only output
events.\et{what are those?}

The identity compiler trivially translates source to target programs.
%
We want to prove that this compiler robustly preserves (modulo the relation
between source and target traces) certain classes of properties. In our
particular setting, since all programs are terminating and therefore all traces
are finite, all trace properties are safety properties.
%
In particular, to prove $\rtcone$ \et{define it}, given $\src{P}$, $\trg{C_T}$ and $\tT{t}$
such that $\ctPmkt{C}{P}{t}$, we need to find $\src{C_S}$ and a related $\tS{s}$
in the source such that $\csPmkt{C}{P}{s}$.
%
\MP{
  notation P and C not defined
}
The source trace $\tS{s}$ is uniquely determined from $\tT{t}$ as the trace that
retains the final result event and removes any preceding target-only output
events.
%
The source context $\src{C_S}$ is obtained by applying a back-translation
function to $\trg{C_T}$ that traverses target expressions and leaves them
unchanged except for the removal of output instructions.
%
It is easy to see that the resulting context exactly the same computational
behavior as its input, without the observational effects of the output
instructions.

Moreover, the same technique serves to prove stronger properties such as those
associated to noninterference, in which $\src{C_S}$ is derived solely from $\src{P}$
and $\trg{C_T}$, and $\tS{s}$ alone can make use of $\tT{t}$. In this setting,
it is already the case that $\src{C_S}$ and $\tS{s}$ depend exclusively on
$\trg{C_T}$ and $\tT{t}$, respectively.
%
\rb{The proper definitions for this are not yet established in the text.}

Given the relation between source and target traces, the induced mapping
$\tilde{\tau}$ interprets a source property as the target property that yields
the same result while producing any trace of target outputs during the
computation. Therefore, proofs about source properties transport easily to the
target language.
%
Conversely, the induced mapping $\tilde{\sigma}$ will often yield an
unsatisfiable proof obligation in the source. In particular, target properties
that do not refer to target-only events will produce equivalent, satisfiable
proof obligations in the source. However, target properties that involve
target-only events---here, (target-level) output events---cannot possibly be
observed in the source and are therefore unprovable.

In the foregoing discussion, for the sake of simplicity, the semantics was not
decorated with control transfer events---from program to context and vice versa.
If these events are available in both source and target, the setting becomes
slightly more interesting\et{slightly...}.
%
To begin, the relation between traces becomes slightly more complicated\et{slightly...}. On the
one hand, a source trace now consists of a finite sequence of pairs of transfer
control events finished by a result event.
%
\rb{At the moment we do not assume one of the program or the context always has
  initial control; it would make the formulation easier.}
%
On the other hand, a target trace obeys this structure and moreover allows its
special output events, but only in the context sections of the trace.

\rb{New trace relation here.}

The compiler and proof technique remain unaltered. Nonetheless, we can make an
interesting observation about the induced mapping $\tilde{\sigma}$ more clearly.
%
\rb{Thinking about proving a target property in the source up to the point where
  the first target-only event appears. These would work as a sort of
  target-level undefined behavior.}

\rb{More languages, etc. Formalization?}

\et{where is this going?}


==> robust_diff_traces.tex <==
% !TEX root = ./rc.tex
\section{Differing Source and Target Trace Models}
\label{sec:Rdifferent-traces}

%\ca{TODO:R maybe look for better title and move somewhere else}
%\ch{Made title better. And this should be indeed at the end of the appendix.}

So far we have assumed that the source and target languages share the
sets of traces and properties.
%
This is a reasonable assumption if observable events are coarse enough
to be common to the source and target language (\EG as it happens
CompCert~\cite{Leroy09}).
%
There are various settings in which this assumption does not hold though:R
\begin{itemize}
\item when values appear in traces and the source and target don't
  share the same notion of values~\cite{PatrignaniG17};
\item when the source language has ``undefined behavior'', which is a
  special event only occurring in source traces, and which leads to
  an arbitrary trace continuation in the target~\cite{Leroy09};
\item when the target language has more events because it is the
  target of multiple source languages;
\item when traces model observations that could become more precise at
  lower levels, \EG because of side-channels like
  timing~\cite{CostanzoSG16};\ch{But with traces formed of such
    leakages even compiler correctness is hopeless~\cite{BartheGL18},
    even more our extensions of it to adversarial contexts!  So maybe
    this is not such a great example after all. The only kind of work
    that could fit here is the one by Zhong Shao~\cite{CostanzoSG16},
    where the source and target observations are different, but still
    equivalent. So started watering this down by adding a ``could'' above.}
\item in general, when there is a big difference between the
  abstractions of the source and target languages.
\end{itemize}

% \MP{ there's other reasons too:R again, the target may talk about more
%   things, because it's a compilation target for multiple languages and
%   the source is a language designed with a specific abstraction in mind. }

% \rb{I would also try to give a general description of causes for the divergence
% and then some examples, like you have now.}
%
\ch{I find this bijection story a confusing digression,
  but would still like to understand why would it be relevant here}%
Using standard set-theoretical arguments we know that, if the two sets of events are both finite or in a bijection,
then so are the sets of traces and properties. In general such a bijection between traces is not constructive,
so that it is interesting to study variants of our criteria handling the discrepancies between trace events.
In this section we focus on \rtp and \pf{\rtp}, leaving a generalization to the remaining criteria as future work.

% \MP{ latex guideline:R the \textbackslash\textbackslash\ is not meant to be used in text, it often breaks things}

In this section, typographic conventions for source and target elements extend
to properties, previously common to both levels. We will denote with \tS{s} and \tT{t} source and
target traces respectively. \ca{any other proposal is welcome, just modify macros in cmd.tex}
%
From a security point of view, \pf{\rtp} captures the fact that if
some $\trg{C_T}$ can mount an attack $\tT{t}$ in the target
language, then the same attack is possible in the source.
%
A natural generalization of \pf{\rtp} requires that the target attack
\tT{t} can be simulated in the source by producing a source trace
\tS{s} that is {\em related} to the target trace \tT{t}.

% \rb{'tries to capture'? Can it fail? This should be a bit clearer.} \ca{changed to just 'captures'}


\begin{definition}[\rtcone] \label{defn:Rrtcone}
Given a relation between source and target traces, $\sim \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$, we define
% \rb{This concept needs a name here, also so we can refer to it later.}
% \ca{done}
\begin{align*}
  \rtcone:R \quad\ \forall\src{P}.~ \forall\trg{C_T}.~ \forall \tT{t}.~ \ctPmkt{C}{P}{t}
         \Rightarrow \mathrel{\exists\src{C_S}\ldotp \exists\tS{s} \sim \tT{t}} \ldotp \csPmkt{C}{P}{s}
\end{align*}
%
\end{definition}


% \vspace{10pt}
%\MP{ don't use arbitrary vspace s, use smallskip / medskip or bigskip, which are more standard :R) }

\smallskip

% \rb{Target properties are not in bold. Introducing trace properties in RTP~
% after RTC~, which inverts the usual order throughout the paper, is potentially
% confusing. If that is changed, the following paragraph also needs to be
% adjusted (let me know if not, so I can reword a bit).}
% \ca{I introduced RTC~ first because it seems easier to explain as a generalization}
As $\pf{\rtp}$, the statement of \rtcone is ``property-free''.
%
In order to bring properties into the picture,
two important questions arise:R
(1) what $\piT{\pi}$ will robustly satisfied in the
target if we have established (\EG by verification) that
some $\src{\pi_S}$ is robustly satisfied in the source, and dually
(2) what is the $\src{\pi_S}$ that must be robustly satisfied in
the source in order to guarantee the robust satisfaction of
a fixed $\piT{\pi}$ we want to obtain in the target.
%
Reflecting this duality, we therefore provide two different
generalizations of $\rtp$ to different source and target traces:R

\begin{definition}[\taurtp and \sigmartp] \label{defn:RRTP}
\  Given an arbitrary pair of mappings between source and target properties,  $\tau :R  2^\src{\ii{Trace}_S} \rightarrow 2^\trg{\ii{Trace}_T}$,
  $~\sigma :R 2^\trg{\ii{Trace}_T} \rightarrow 2^\src{\ii{Trace}_S} $ we define:R
  % \rb{Again, give names to these!}
%
%  \MP{ while their types are, they are not necessarily the inverse of one another. }
%  \MP{ i think it's less confusing if you write the two definitions instead of just one like now. }
%
  % \rb{These equations can break in annoying places, could we do something about
  % the spacing?}

  \begin{align*}
    \taurtp:R \quad
    \forall \src{\pi_S} \in 2^\src{\ii{Trace}_S}.~\forall\src{P}.~
    &
      (\forall\src{C_S}~\tS{s} \ldotp
      \mathrel{\src{C_S\hole{P} \sem}} \tS{s} \Rightarrow \tS{s}\in\src{\pi_S})
      \Rightarrow
    \\
    &
      (\forall \trg{C_T}~\tT{t} \ldotp
      \mathrel{\trg{C_T\hole{\cmp{P}} \sem}} \tT{t} \Rightarrow \tT{t}\in\tau(\src{\pi_S}))
    \\
    \\
    \sigmartp:R \quad
    \forall \piT{\pi} \in 2^\trg{\ii{Trace}_T}.~\forall\src{P}.~
    &
      (\forall\src{C_S}~ \tS{s} \ldotp
      \mathrel{\src{C_S\hole{P} \sem}} \tS{s} \Rightarrow \tS{s}\in \sigma(\piT{\pi}))
      \Rightarrow
    \\
    &
      (\forall \trg{C_T}~\tT{t} \ldotp
      \mathrel{\trg{C_T\hole{\cmp{P}} \sem}} \tT{t} \Rightarrow \tT{t}\in\piT{\pi})
\end{align*}
%
\end{definition}
%
% \vskip 1cm
\bigskip
%
% \rb{This needs a lead-in to understand why they will be useful. What are we
% trying to get to?} \ca{added something}
The mapping $\tau$ fixes an interpretation of source properties in the
target language, while $\sigma$ fixes an interpretation of target
properties in the source language.
%
For example, $\tau$ tells us how to
interpret the source property \emph{``The program does not encounter an undefined behavior"} in a target
language with no symbol for undefined behavior in it events alphabet.

\ch{We are still badly missing intuition why a Galois connection is a
  reasonable thing to require/expect here. Simply making the proof
  below work does not count as intuition! Also we don't yet have an
  explanation why this Galois connection goes in the opposite
  direction compared to what the intuition would say.}

We are going to show, in \Cref{thm:Rgalois}, that certain conditions on $\tau$ and $\sigma$ provide the equivalence
of \taurtp and \sigmartp. First of all let us recall the definition and a useful characterization of \emph{Galois connections} \cite{CousotCousot77-1}.
% \ca{Does this reference work?}
%that will be useful later on.


\begin{definition}[Galois connection] Let $(X, \leq)$ and $(Y, \sqsubseteq)$ be two posets.
  A pair of maps, $\alpha:R X \to Y$, $\gamma:R Y \to X$ is a Galois connection \ii{iff}
  it satisfies the following \emph{adjunction law}:R
%
                   \begin{equation*}
                     \forall x \in X. ~ \forall y \in Y. ~ \alpha(x) \sqsubseteq y \iff x \leq \gamma(y)
                   \end{equation*}
%
$\alpha$ is referred to as the \emph{lower adjoint} and $\gamma$ as the \emph{upper adjoint}.
We will often write  $\alpha:R (X, \leq) \leftrightarrows (Y, \sqsubseteq) :R\gamma$ to denote a Galois connection.
%
\end{definition}

\begin{lemma}[Characteristic property of Galois connections] \label{lem:RchG}
  % \rb{Have you used the double arrow notation before? If not, one should do so,
  % and use this name to lead the statement of the lemma.} \ca{fixed}
  $\alpha:R (X, \leq) \leftrightarrows (Y, \sqsubseteq) :R\gamma$ is a Galois connection if and only if $\alpha, \gamma$ are monotone and
  they satisfy the following properties:R
  % \rb{Briefly name these. Is it a property or two properties?} \ca{added numbers}
  \begin{align*}
   i)& \quad \forall x \in X.  ~ x \leq \gamma(\alpha (x)) \\
   ii)& \quad \forall y \in Y. ~ \alpha(\gamma (y)) \sqsubseteq y
  \end{align*}
%
\end{lemma}
%
\bigskip
%
\ch{zero intuition here}%
It turns out that if $\tau \leftrightarrows \sigma$ is a Galois connection, the two
criteria in \Cref{defn:RRTP} are equivalent.
% \rb{Give the criteria by name. Also establish the convention of using one for
% source to target and vice versa, so there is no confusion *and* it is clear
% that they are not going in the same direction (above?). I think in this lead-in
% the clearest thing is to not mention tau and sigma, which are in the statement
% just below, and talk in general terms.}
\ca{TODO:R not sure if I fully integrated RB comments}

\begin{theorem}[\taurtp and \sigmartp coincide] \label{thm:Rgalois}

 If  $\tau :R  (2^\src{\ii{Trace}_S}, \subseteq) \rightleftarrows (2^\trg{\ii{Trace}_T}, \subseteq) :R \sigma $
 is a Galois connection, with $\tau$ its lower adjoint and $\sigma$ its upper adjoint, then
 $ \taurtp \iff \sigmartp $.

\end{theorem}
%\MP{ i think we should define a galois connection for the reader, or at least point to a reference. }
%\ca{TODO:R add defn of Galois Connection and some charcterization used}

\begin{proof}
  As a preliminary remark observe that, both in the source and target,
  if a program robustly satisfies a property $\pi$, then it robustly satisfies every extension
  $\pi' \supseteq \pi$. Using this we prove the claim of the theorem:R
\ch{Please make it more explicit below where the remark above
  and the precise conditions of the Galois connection are used:R}

  ($\Rightarrow$)\quad Assume \taurtp and that $\src{P}$ robustly satisfies $\sigma(\piT{\pi})$. Apply
  \taurtp to $\src{P}$ and $\sigma(\piT{\pi})$ and deduce that $\cmp{P}$ robustly satisfies
  $\tau(\sigma (\piT{\pi})) \subseteq \piT{\pi}$.

  ($\Leftarrow$)\quad Assume \sigmartp and that $\src{P}$ robustly
  satisfies $\src{\pi_S} \subseteq \sigma( \tau (\src{\pi_S} ) )$. Apply \sigmartp to $\src{P}$
  and $\sigma( \tau (\src{\pi_S} ) )$ deducing $\cmp{P}$ that robustly satisfies $\tau (\src{\pi_S} )$.
\end{proof}

\ch{Does the other direction of the theorem above hold?  Can we obtain
  that $\tau$ and $\sigma $ form a Galois connection from a proof that
  $ \taurtp \iff \sigmartp $?}

% \rb{So is this going both directions? Clarify with above. This is a bit
%     confusing to read, for me.}
% \ca{tried to clarify}
So far we discussed how to generalize the criterion for the
preservation of robust satisfaction of all trace properties, $\rtp$.
%
We showed that it is possible to start either from the property-free
characterization $\pf{\rtp}$ and a relation between source and target
traces (\Cref{defn:Rrtcone}), or from $\rtp$ and an interpretation
of properties of one language into the other (\Cref{defn:RRTP}).
%
Below we investigate the relation between \rtcone and
\taurtp/\sigmartp.  In \Cref{sec:Rtilde} we define two natural mappings
$\tilde{\tau}$, $\tilde{\sigma}$ starting from a given relation $\sim$
and discuss under which conditions the three criteria presented are
all equivalent.
%
These extra conditions may restrict the class of target properties for
which a one can use source-level reasoning, even when a secure
compilation chain is available.
%
In \Cref{sec:Rconnection} we start from a Galois connection
$\tau \rightleftarrows \sigma$ and define a relation that ensures the
equivalence.


% \ca{good titles are welcome}
\subsection{Deriving Property Mappings from a Relation} \label{sec:Rtilde}

In this section we show how a relation $\sim$ between source and target traces induces a pair of mappings from properties of one language
to properties of the other language. We specialize \Cref{defn:RRTP} with such interpretation and show that one of the criteria is
equivalent to $\rtcone$ with no extra assumption (\Cref{thm:Rrtprtc}), while in general the other one is stronger (\Cref{lem:Rleft}).

\begin{definition}[Induced mappings] \label{defn:Rtilde}

  Let  $\sim \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$

  \begin{align*}
    \tilde{\sigma} & = \lambda ~\piT{\pi}. ~ \myset{ \tS{s} }{ \exists \tT{t} \in \piT{\pi}. ~ \tS{s} \sim \tT{t} } \\
    \tilde{\tau}   & = \lambda ~\src{\pi_S}. ~ \myset{ \tT{t} }{ \exists \tS{s} \in \src{\pi_S}. ~ \tS{s} \sim \tT{t} }
  \end{align*}

We denote with {\tildetaurtp}, \tildesigmartp the criteria in
\Cref{defn:RRTP} for $\tilde{\tau}$ and $\tilde{\sigma}$ respectively.

\end{definition}

\begin{theorem}[\tildetaurtp and \rtcone always coincide] \label{thm:Rrtprtc}
  Let  $\sim \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$, then $\tildetaurtp \iff \rtcone$.
\end{theorem}

%\MP{ at this point i would assume that i can reuse the general facts proven before about sigma (not sigma hat) and tau, why is it not the case? should i need extra assumptions on the tilde to prove things then just based on the old proofs?}
%\ca{in general $\tilde{\tau}, \tilde{\sigma}$ are not a galois connection, so you cannot apply \Cref{thm:Rgalois}}

% \rb{Maybe this is OK, but the proof is a little too high-level for me, in that
% it takes so many details for granted that it isn't easy to follow.}
\begin{proof}
($\Rightarrow$)\quad Assume \tildetaurtp in contrapositive form and assume $\mathrel{\trg{C_T\hole{\cmp{P}} \sem}} \tT{t}$.
We can apply \tildetaurtp to $\src{P}$ and $\src{\pi_S} \equiv \myset{\tS{s}}{\tS{s} \not\sim \tT{t}}$.
If it is non-empty, $\tilde{\tau}(\src{\pi_S})$ contains $\tT{t}$,
in both cases $\cmp{P}$ does not robustly satisfy it. % \rb{What both cases? Empty and non-empty?}
We therefore deduce $\exists \src{C_S}\exists \tS{s}. ~\mathrel{\src{C_S\hole{P} \sem}} \tS{s} $ and $\tS{s} \notin \src{\pi_S}$, from which $\tS{s} \sim \tT{t}$.

($\Leftarrow$)\quad Assume \rtcone and that for $\src{P}, \src{\pi_S}$ there exists $\trg{C_T}$
such that $\mathrel{\trg{C_T\hole{\cmp{P}} \sem}} \tT{t}$ with $\tT{t} \notin \tilde{\tau}(\src{\pi_S})$.
Apply \rtcone and deduce $\mathrel{\exists\src{C_S}\ldotp \exists\tS{s} \sim \tT{t} \ldotp\src{C_S\hole{P}\sem}} \tS{s}$. If $\tS{s} \in \src{\pi_S}$,
then $\tT{t} \in \tilde{\tau}(\src{\pi_S})$, which is a contradiction and therefore $\tS{s} \notin \src{\pi_S}$.
\end{proof}

Note that \Cref{thm:Rrtprtc} does not require any extra assumptions.
On the other hand, in general \tildesigmartp and \rtcone are not equivalent (as shown by \Cref{ex:Rlength} below),
although the equivalence can be shown under some extra conditions,
which are subsumed by the adjunction law of the Galois connection.\ch{Is one
  of the conditions in \autoref{lem:RchG} enough?}

\begin{lemma}[\tildesigmartp stronger than \rtcone]\label{lem:Rleft}
 Let  $\sim \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$ be such that $ \forall \tS{s}. ~\exists \tT{t}. ~ \tS{s} \sim \tT{t}$,
 then \sigmartp $\Rightarrow$ \rtcone.
\end{lemma}

\begin{proof}
  Assume  $\mathrel{\trg{C_T\hole{\cmp{P}} \sem}} \tT{t}$, and consider
  the target property $\piT{\pi} = \myset{\trg{t_T'}}{\trg{t_T'} \neq \tT{t}}$. By \sigmartp deduce
  $\mathrel{\src{C_S\hole{P} \sem}} \tS{s}$ for some $\src{C_S}$ and some $\tS{s} \not\in \tilde{\sigma}(\piT{\pi})$.
  This means that $\tS{s}$ is not related to target traces different from $\tT{t}$, and from our hypothesis we deduce $\tS{s} \sim \tT{t}$,
  which concludes the proof.
\end{proof}

We introduce the following, weaker variant of \tildesigmartp, which will be shown to follow from \rtcone.
% \rb{Definition?}

\begin{definition}[Weak $\tildesigmartp$] \label{def:Rweaker}

  Let  $\sim \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$,

  \begin{align*}
    \weaktilde \equiv \quad
    \forall \piT{\pi} \in \mathcal{G}.~\forall\src{P}.~
    &
      (\forall\src{C_S}~ \tS{s} \ldotp
      \mathrel{\src{C_S\hole{P} \sem}} \tS{s} \Rightarrow \tS{s}\in \sigma(\piT{\pi}))
      \Rightarrow
    \\
    &
      (\forall \trg{C_T}~\tT{t} \ldotp
      \mathrel{\trg{C_T\hole{\cmp{P}} \sem}} \tT{t} \Rightarrow \tT{t}\in\piT{\pi})
  \end{align*}

\bigskip

where  $ \mathcal{G} = \{ \piT{\pi} | ~ \forall \trg{t_1} \trg{t_2} \tS{s}. ~
                                \tS{s} \sim \trg{t_1} \wedge \tS{s} \sim \trg{t_2} \Rightarrow
                                (\trg{t_1} \in \piT{\pi} \iff \trg{t_2} \in \piT{\pi}) \} $

\end{definition}
% \vspace{10pt}
% \MP{ noneeee, add skips, not vspaces :R) }
%
\bigskip
It is possible to show, by straightforward manipulations, that the class $\mathcal{G}$ coincides with the class of all
properties  $\piT{\pi}$ such that $\tilde{\tau} (\tilde{\sigma} (\piT{\pi})) \subseteq \piT{\pi}$.

\begin{lemma}[\rtcone stronger than \weaktilde] \label{lem:Rright}
  Let  $\sim \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$, \rtcone $\Rightarrow$ \weaktilde.
\end{lemma}

\begin{proof}
 We prove the contrapositive of {\weaktilde}. Assume $\mathrel{\trg{C_T\hole{\cmp{P}} \sem}} \tT{t}$ with $\tT{t} \not\in \piT{\pi}$,
 for an arbitrary $\piT{\pi} \in \mathcal{G}$. Applying \rtcone we deduce $\mathrel{\src{C_S\hole{P} \sem}} \tS{s}$
 for some $\src{C_S}$ and some $\tS{s} \sim \tT{t}$.  We just need to show that $\tS{s} \not\in \tilde{\sigma}(\piT{\pi})$.
 If $\tS{s} \in \tilde{\sigma}(\piT{\pi})$
 then  $\tT{t} \in \tilde{\tau}(\{ \tS{s} \}) \subseteq \tilde{\tau}(\tilde{\sigma}(\piT{\pi})) \subseteq \piT{\pi}$,
 a contradiction.
\end{proof}

When the two maps form a Galois connection it is possible to show that every source trace is related to some target trace,
and that $\mathcal{G} = 2^\trg{\ii{Trace}_T}$, so that \tildesigmartp and its weaker variant coincide.

\begin{corollary}[\tildetaurtp, \rtcone and \tildesigmartp all coincide]\label{cor:R3eq}
   If  $\tilde{\tau} \rightleftarrows \tilde{\sigma}$ is a Galois connection then
   $\tildetaurtp \iff \rtcone \iff \tildesigmartp$.
\end{corollary}

\begin{proof}
  The thesis\ch{??? please be explicit what!}
  follows from \Cref{thm:Rgalois} and \Cref{thm:Rrtprtc}, we also propose a direct proof
  that shows the adjunction law ensures that $\forall \tS{s}. ~ \exists \tT{t}. ~ \tS{s} \sim \tT{t}$,
  and that $\mathcal{G} = 2^{\trg{\ii{Trace}_T}}$.

  Let $\tS{s}$ be a source trace, trivially $\tilde{\tau}(\{ \tS{s} \}) \subseteq \tilde{\tau}(\{ \tS{s} \})$
  so that by the adjunction law we deduce $ \{ \tS{s} \} \subseteq \tilde{\sigma}(\tilde{\tau}(\{ \tS{s} \}))$,
  that means there exists some $\tT{t}$ such that $\tS{s} \sim \tT{t}$.

  Finally the characteristic property of Galois connections in \Cref{lem:RchG},
  $\forall \piT{\pi}. ~ \tilde{\tau} (\tilde{\sigma} (\piT{\pi})) \subseteq \piT{\pi}$.
  Thesis\ch{????? please be explicit what!}
  hence follows  from \Cref{lem:Rleft} and \Cref{lem:Rright}.
\end{proof}

% \MP{ don't you mean RTPsigma weak here? i don't follow the text otherwise. }
% \ca{If $\tilde{\tau}, \tilde{\sigma}$ is a Galois connection then \weaktilde is equivalent to \tildesigmartp}

\smallskip

\textbf{NEW} \\
\ca{TODO:R Understand where to place this and if and how structure this document} \\

So far we know that, independently from the relation chosen, $\tildetaurtp \iff \rtcone$,
\Cref{ex:Rlength} however shows $\rtcone$ is not in general equivalent to $\tildesigmartp$.
A sufficient condition for $\tildetaurtp \iff \rtcone \iff \tildesigmartp$ is that $\tilde{\tau} \rightleftarrows \tilde{\sigma}$
is a Galois connection, \Cref{cor:R3eq}. This suggests that replacing $\tilde{\sigma}$ with the upper adjoint of $\tilde{\tau}$, say $\tilde{\gamma}$,
and defining $\rtpdiff{\tilde{\gamma}}$ in the obvious way, the equivalence $\tildetaurtp \iff \rtcone \iff \rtpdiff{\tilde{\gamma}}$
holds (\CoqSymbol branch diff\_traces, file SigmaTau.v Lemma $\tau$RTP\_$\gamma$RTP). The upper adjoint
of $\tilde{\tau}$ always exists (\CoqSymbol Lemma $\gamma'$\_upper\_adjoint\_$\tau'$) and is defined as following
%
\begin{equation*}
  \tilde{\gamma} = \lambda ~\piT{\pi}. ~ \myset{ \tS{s} }{ \forall \tT{t}. ~\tS{s} \sim \tT{t} \Rightarrow \tT{t} \in \piT{\pi}}
\end{equation*}

\smallskip

%
$\tilde{\gamma}$ coincides with $\tilde{\sigma}$ if and only if the relation $\sim$ is a total function
from source to target traces (\CoqSymbol Theorem $\sigma'$\_$\tau'$\_adjoint\_iff), this is not the case of \Cref{ex:Rlength}.
\ca{TODO:R explain why}
%
In the study of preservation of robust satisfaction of classes of (hyper)properties we will therefore
consider $\tilde{\gamma}$ rather than $\tilde{\sigma}$. \\
%
\ca{Probably the set $\mathcal{G}$ is the set on which $\tilde{\gamma}$ and $\tilde{\sigma}$ coincide (to be checked)}
\textbf{WEN}


% \ca{good titles are welcome}
\subsection{Deriving a Relation from Maps} \label{sec:Rconnection}

% \MP{ please, give a bit more intuition. now, we're building the relation timse starting from the adjuncts. before, we were building the adjuncts based on the relation.
%   You should
%   1) use subsections to split this
%   2) write a common header that explains what's going to happen and
%   3) explain why these two approaches are interesting (because they are! they model different approaches to formalising security properties!)
% }

% TODO:R give a look to https:R//ncatlab.org/nlab/show/Galois+connection#InducedFromARelation

In this section, given a Galois connection between source and target
properties we define a relation over source and target traces ensuring the
equivalence between \rtcone and \sigmartp and \taurtp.

\begin{definition}[Induced relation] \label{defn:Rrelation}
  Let $\tau :R  2^\src{\ii{Trace}_S} \rightarrow 2^\trg{\ii{Trace}_T}$ and  $~\sigma :R 2^\trg{\ii{Trace}_T} \rightarrow 2^\src{\ii{Trace}_S}$, define
   $\simst \,\subseteq \src{\ii{Trace}_S} \times \trg{\ii{Trace}_T}$ as following

  \begin{equation*}
    \tS{s} \simst \tT{t} \iff \tT{t} \in \tau(\{ \tS{s} \})
  \end{equation*}

\end{definition}

% \vspace{10pt}
\medskip

\begin{theorem}[\taurtp, \rtctwo and \sigmartp all coincide]
  If  $\tau \rightleftarrows \sigma$ is a Galois connection then
          $$ \taurtp \iff  \rtctwo \iff \sigmartp $$
\end{theorem}

% \MP{ apart from the missing ref, many theorems don't have names. please add names, it helps readers a lot (even when the statements are very simple, yes)}

\begin{proof}
  It suffices to show the equivalence between \rtctwo and \sigmartp, then by \Cref{thm:Rgalois}
  we get the other equivalence.

  ($\Rightarrow$)\quad
  Assume \rtctwo and assume that $\mathrel{\trg{C_T\hole{\cmp{P}} \sem}} \tT{t}$ and
  $\tT{t} \notin \piT{\pi}$ for some $\src{P}$ and some $\piT{\pi}$.
  By \rtctwo deduce $\mathrel{\src{C_S\hole{P} \sem}} \tS{s}$ for some $\src{C_S}$ and
  some $\tS{s}$ such that $\tT{t} \in \tau(\{ \tS{s} \} )$.
  It now suffices to show that $\tS{s} \notin \sigma(\{ \piT{\pi}\})$.
  If $\tS{s} \in \sigma(\{ \piT{\pi}\})$, by the adjunction law we get
  $\tau(\{ \tS{s} \}) \subseteq \piT{\pi}$ and hence $\tT{t} \in \piT{\pi}$, a contradiction.

  ($\Leftarrow$)\quad
  Assume \sigmartp and $\mathrel{\trg{C_T\hole{\cmp{P}} \sem}} \tT{t}$
  for some $\src{P}$ and some $\tT{t}$.
  By \sigmartp applied to  $\piT{\pi} \equiv \{ \trg{t'} | ~\trg{t'} \neq \tT{t} \}$
  deduce the existence of some $\src{C_S}$ such that $\mathrel{\src{C_S\hole{P} \sem} \tS{s}}$
  and $\tS{s} \notin \sigma(\piT{\pi})$. We still need to show that $\tT{t} \in \tau(\{ \tS{s} \})$.
  By $\tS{s} \notin \sigma(\piT{\pi})$ and the adjunction law deduce
  $\tau(\{ \tS{s} \}) \not\subseteq \piT{\pi}$ that implies $\tau(\{ \tS{s} \}) = \{ \tT{t} \}$.
  \MP{ it'd be nice to have REFS for stuff like the adjunct law, so you can refer to them and the reader can more easily follow the proof.
  You can use command :R thmref for that.}
\end{proof}

\subsection{Unsafe Languages and Side-Channels} \label{sec:Rexamples}

In this section we show how the criteria above deal with two
interesting case studies.
%
In \Cref{ex:Rundef} we consider an unsafe source
language~\cite{AbateABEFHLPST18}, while in \Cref{ex:Rlength} a timer is
available to measure time spent for computations of target programs.
%
To model this, in the first case we assume the set of source events
contains a special symbol denoting that the program encountered an
\emph{undefined behavior}~\cite{Leroy09}.
%
In the second case we equip target traces with a natural number,
intuitively denoting the number of time units, e.g. ms, needed by the
program to produce the trace.
%
In both cases source and target traces differ, but are related by
some relation $\sim$.
%
We explain the guarantees an \rtcone compilation chain provides, and
discuss whether and how \tildetaurtp and \tildesigmartp match the same guarantees.

%  \MP{ of what? for what purpose? this should perhaps be another subsection}
% We leave the source and target languages abstract and focus on traces and properties.

\begin{example}[Relating traces when the source has undefined behaviour] \label{ex:Rundef}
Let $\Sigma$ be some set of events and an $\eundef$ a symbol not contained by $\Sigma$. Assume observable events in the source
are $\src{\Sigma} = \Sigma \cup \{ \eundef \}$, while in the target $\trg{\Sigma} = \Sigma$.
%
If a source program encounters an undefined behavior
then the source semantics immediately terminates its computation, so
that source traces can exhibit the symbol $\eundef$ only at the end
of a (finite) trace.
%
Notice that properties, traces and finite prefixes in the target are all valid properties, traces and
finite prefixes in the source.

We say that a target trace \emph{refines} a source trace, and write $\tS{s} \sim \tT{t}$
\emph{iff} $\tS{s} = \tT{t} \vee \exists m \leq \tT{t}. ~ \tS{s} = {m} :R:R \eundef$.
%
\rtcone{} holds for a compilation chain if, whenever a trace $\tT{t}$ is produced in some target context
by some $\cmp{P}$, then there is a source context in which $\src{P}$ can either faithfully
reproduce $\tT{t}$ or encounter an undefined behavior while trying.
%
\tildesigmartp holds if, in order to claim
$\cmp{P}$ robustly satisfies a target property, it suffices to show
that computations of $\src{P}$ satisfy the same property or stop
prematurely exhibiting an undefined behavior.
% \rb{Meaning P compiled?} \ca{it's \src{P} because the simulation is
% meant to be in the source}
%
Finally, \tildetaurtp holds if whenever a source property is robustly satisfied,
a certain \emph{refinement}
of the same property is robustly satisfied in the target.
% \rb{I think this is a little more concrete than the phrasing leads to believe.}
%
The equivalence of these three criteria can be rigorously checked by simply unfolding our definitions
of $\tilde{\tau}$ and $\tilde{\sigma}$. Indeed,
%
\begin{align*}
  \tilde{\tau}(\piS{\pi}) &=  \myset{\tT{t}}{\tT{t} \in \piS{\pi}} \cup \myset{\tT{t}}{\exists m \leq \tT{t}. ~ m :R:R \eundef \in \piS{\pi}} \\
  \tilde{\sigma}(\piT{\pi}) &= \piT{\pi} \cup \myset{ m :R:R \eundef}{ \exists \tT{t} \in \piT{\pi}. ~ m \leq \tT{t}}
\end{align*}
%
Notice that every source trace is related to some target trace and that for an arbitrary $\piT{\pi}$, $\tilde{\tau}(\tilde{\sigma} (\piT{\pi})) = \piT{\pi}$,
so that \tildesigmartp coincides with its weaker variant and
$\tildetaurtp \iff \rtcone \iff \tildesigmartp$.
\end{example}

\begin{example}[With side-channels target traces are more informative than source ones] \label{ex:Rlength}
In this example source and target share the same set of observable events, but we assume a timer is available in  the target.
To model this we equip source traces with a natural number that intuitively gives us an estimation of the time needed to
produce the trace.

In more detail, let $\src{\ii{Trace}_S}$ denote the set of traces in the source, $\trg{\ii{Trace}_T} = \src{\ii{Trace}_S} \times (\mathbb{N} \cup \{ \omega \})$.
Write  $\trg{W_T \leadsto}_n ~\tS{s}$ to denote that $\trg{W_T}$ produces $\tS{s}$ in at most $n$ units of time, e.g. ms.
If $n = \omega$ then we mean that $\trg{W_T}$ produces $\tS{s}$ in an arbitrary, maybe infinite, amount of time.
Define the relation $\sim$ as follows:R

% \rb{I think this may benefit from a bit of explanation on the second case.}
\ch{I find the second conjunct below silly.
  And it's still not even explained. How about removing it?
  Or do the results below depend on it? If so it's fishy.}
\begin{center}
  $\tS{s} \sim \tT{t}$ \emph{iff} $\exists n. ~\tT{t} = (\tS{s}, n) \wedge ~\exists \trg{W_T}. ~ \trg{W_T \leadsto}_n ~\tS{s}$.
% in less than $n$ units of time
  % if $n \in \mathbb{N}$, in arbitrary time if $n = \omega$.
\end{center}
%
Notice that a trace produced by some target program is
related to the source trace that
simply ``forgets'' the time spent in the computation.
\rtcone{} requires that, if an attack can be mounted at the target level, the same attack can be
simulated, no matter in how much time, in the source.
%
\ch{I would start by explaining that $\tilde{\sigma}$ and $\tilde{\tau}$ do not
  form a Galois connection.}%
%
It is easy to show that for the set of properties $\mathcal{G}$ we get
from \autoref{def:Rweaker}\ch{Re-Explain the intuition of this set}
$\mathcal{G} \neq 2^{\trg{Trace}}$ and
that \weaktilde{} is indeed weaker than $\tildesigmartp.$
Intuitively a $\piT{\pi}$ may contain spurious pairs $(\tS{s}, n)$,
where $n$ is not large enough to represent a sufficient amount of execution time, and $\tilde{\sigma}$ removes all of them.
%
For instance let $\tS{s}$ be an infinite trace, $\tilde{\sigma}(\{ (\tS{s}, 0)\}) = \emptyset$ because
there is no way to produce an infinite trace in $0$ units of time.
%
\weaktilde{} tells us that $\cmp{P}$ robustly
satisfies $\{ (\tS{s}, 0)\}$ if $\src{P}$ robustly satisfies the empty property, which is not possible.
\end{example}

\ch{So what's the conclusion of this example? If I care about side-channels,
  should I not use any of these definitions? Os should I only give up on
  $\weaktilde$?}


==> texdirectives.tex <==
\draftfalse\anonfalse\camerafalse\appendixtrue


==> two_dot_one.tex <==
\subsection{Compiler Correctness}

\et{does not connect with intro presentation}
\jt{I guess we should remove this section}

Compiler correctness is often formulated through a refinement relation between 
the behaviors of the compiled program and 
the original one \ca{cite Amal's paper}. For whole programs $W$ and for a fixed notion of refinement, $\sqsubseteq$ 
compiler correctness is therefore defined as following. 

\begin{definition}[Compiler Correctness Scheme]
  
  A compilation chain $\downarrow$ is correct for $\sqsubseteq$ if an only $\ccomp$ holds for $\downarrow$.
 
  \begin{equation*}
   \ccomp \equiv \forall \src{W}. ~ \cmp{W} \sqsubseteq \src{W}  
  \end{equation*}
  
\end{definition}
%
When program behaviors, denoted by $\ii{beh}(W)$ are modeled as sets of traces the refinement is 
usually implemented as set inclusion and a common set of traces is used to model the executions of both source and
target traces \ca{cite }. When $\sqsubseteq$ is $\subseteq$, $\ccomp$ is called \emph{backward} compiler correctness, 
if $\sqsubseteq$ is $\supseteq$, \emph{forward} compiler correctness. Finally if $\sqsubseteq$ is just set equality,
so that we have both backward and forward correctness, we call $\ccomp$ \emph{hyper} correctness.
 \ca{Is hyper correctness ok? It should suggest the equivalence with hyperproperty preservation}
%
%
\begin{definition}[Backward, Forward, Hyper Correctness] \label{defn:traceCC}

   A compilation chain $\downarrow$ is \emph{backward} (\emph{forward}) (\emph{hyper})
   correct  if an only $\pf{\traceP}$ ($\pf{\traceP}_{\ii{fwd}}$) ($\pf{\hyperP}$) holds for $\downarrow$.

  \begin{align*}
    \pf{\traceP}  \equiv \forall \src{W}. ~ \ii{beh}(\cmp{W}) \subseteq \ii{beh}(\src{W}) \\ 
    \pf{\traceP}_{\ii{fwd}}  \equiv \forall \src{W}. ~ \ii{beh}(\cmp{W}) \supseteq \ii{beh}(\src{W}) \\ 
    \pf{\hyperP}  \equiv \forall \src{W}. ~ \ii{beh}(\cmp{W}) = \ii{beh}(\src{W})
  \end{align*}
  
\end{definition}
%
In this work we are interested in backward compiler correctness and in it equivalent formulation in terms
of preservation of all semantic properties of programs through compilation \ca{cite... who was the first showing this equivalence?}. 
When program behaviors are modeled as sets of traces, semantics properties are usually represented as sets of traces
 (\emph{trace properties}), or sets of sets of traces (\emph{hyperproperties}) \cite{ClarksonS10}. 
A program $W$ satisfies a trace property $\pi$, written $W \models \pi$, if the set of traces denoting its behaviors, $\ii{beh}(W)$ is a subset of the
property considered, $\ii{beh}(W) \subseteq \pi$. $W$ satisfies a hyperproperty $H$ if $\ii{beh}(W) \in H$, we still write $W \models H$ and specify
the type of $\pi, H$ in case it is not clear from the context.  \ca{maybe we should specify that we adopt the notion of hyperproperty
  satisfaction from \cite{ClarksonS10}, there is paper called ``Hyperhierarchy of semantics'' (that is the hyperproperty version of a paper by Cousot) 
  where maybe other choices are described (but I did not read it) }. 

\begin{definition}[Trace Properties and Hyperproperties Preservation] 
  A compilation chain $\downarrow$ preserves all trace properties if an only if
  $\traceP$ holds for $\downarrow$.
%
  A compilation chain $\downarrow$ preserves all hyperproperties if an only if
  $\hyperP$ holds for $\downarrow$.
  
  \begin{align*}
    \traceP & \equiv \forall \pi \in \prop ~\forall \src{W}. ~ \src{W} \models \pi \Rightarrow \cmp{W} \models \pi \\ 
    \hyperP & \equiv \forall H \in 2^{\prop} ~\forall \src{W}. ~ \src{W} \models H \Rightarrow \cmp{W} \models H 
  \end{align*}

\ca{I would go for (ET proposal) $\mathcal{P}(\_)$ rather than $2^{(\_)}$ } 

\end{definition}
\et{shouldn't TP be TPP (Trace Properties Preservation)?}
\et{likewise HP be HPP?}

